A Unified Credit Expansion Theory on Housing Cycle: Causal Evidence for Within- and Cross-Metro Patterns in the Prior, Boom, Bust, and Recovery Periods

During the 1999-2019 U.S. housing cycle, three empirical facts present a puzzle: in the boom period, the correlation between income growth and mortgage growth is (1) negative across ZIP codes within a metropolitan area, but (2) positive across metropolitan areas, and (3) the metropolitan areas that experience the worst bust also show the strongest recovery. I develop a unified credit expansion theory that explains both within- and cross-metro patterns in the prior, boom, bust, and recovery periods (including the three facts above) and generates new testable implications of ``double differences" (cross ZIP codes and cross metros) for the four periods. Following the idea of ``Economic Base Theory", I construct local economic exposure to net export growth as the driving force of local economy and credit expansion. For the identification strategy, I use a new instrumental variable approach from the International trade literature for the following empirical results. First, I show that high-net-export-growth metros experience a stronger boom-bust-recovery housing cycle due to credit expansion in private-label mortgages (PLMs), rather than in government-sponsored enterprise mortgages (GSEMs), because only the former can legally respond to local economic conditions. Second, for the ``double differences", I define a low-minus-high (LMH) factor as the private-label mortgage (and house price) growth in low-income ZIP codes minus that in high-income ZIP codes within the same metropolitan area. I show that this low-minus-high factor (as a measure of credit expansion) in the high-net-export-growth metros is more positive during the boom period, more negative during the bust period, and slightly more positive in the recovery period than in the low-net-export-growth metros. Lastly, I employ five tests to demonstrate that ``speculation" is unlikely to play a dominant role in this housing cycle.

==> Old/Empirical.Preliminary.tex <==
%------------------------------------------------------------
%------------------------------------------------------------
%\clearpage
%------------------------------------------------------------
%------------------------------------------------------------
\subsection{Empirical: Verification Tests}\label{subsec:NEG_LocalEconConditions}



In this section,  I first verify the assumption that net export growth cause a differential higher increase in local employment growth, household income growth, and population growth in the HNEG areas. This assumption is based on the economic base theory and links the causal relation between net export growth to credit expansion in PLM. The growth in employment, household income, and population are three channels through which net export growth induces credit expansion in PLM from 2002 to 2006.  I conduct regression with the following specifications. 
%\vspace{-3mm}
\begin{equation}\label{equ:LocalEconCond_reg_NEG}
    \triangle_{92,06} Ln(LocalEconConditions_{c}) = \beta * \triangle_{92,06} NEP_{m} + \gamma* \bm{Controls_{c}} + \alpha + \epsilon_{c}
\end{equation}
$\triangle_{92,06} Ln(LocalEconConditions_{c})$ represents the growth of local economic condition at the county $c$, which can be employment, household income, and population. We use the gravity-model-based instrumental variable ($\triangle_{92,06}givNEP_{m}$) as IV for $\triangle_{92,06}NEP_{m}$. 


\comment{We include control variables at county $c$ only in the year 1992, which prevents any impact from net export growth. To take consideration of county size, regression is weighted by the natural logarithm of the number of households in 1992. Logarithms rather than the absolute number of households are chosen to prevent regression results from being dominated by a few super-populous counties. To take into account that households might commute to work across counties within a metropolitan area, I measure net export growth in the metropolitan area.\footnote{According to US Census, "the general concept of a metropolitan statistical area is that of a core area containing a substantial population nucleus, together with adjacent communities having a high degree of economic and social integration with that core." (\url{https://www.census.gov/programs-surveys/metro-micro/about.html}} Additionally, I cluster Standard errors at the metropolitan area (MA) level.
} % end of comment





%------------------------------------------------------------
%\subsection{Net Export and Employment Growth}
%------------------------------------------------------------
\subsubsection{Net Export and Employment Growth}

In this test, I use the ratio of total (excluding construction) employment to the working-age population (age 15-64) because I want to avoid the impact of mortgage credit on employment. 

Table (\ref{table:BEATotExConstEmp.D92t06.4Reg}) reports OLS, reduced-form, second stage, and first stage of the results of employment growth in panels A, B, C, and D. First, panel A column (1) shows the positive and significant impact of net export growth (92-06, annualized) on total (excluding construction) employment share growth (92-06, annualized), without any control. Through columns (2) to (4), the estimates show that the OLS coefficient of the next export growth is almost unaffected by the inclusion of the number of households, household income, and number of housing units in 1992. Panel B reports the reduced-form estimates and shows that gravity-model-based net export growth increases household income growth. This significant impact is quite stable to the inclusion of various controls. 

First-stage estimates in panel D show that the strong positive correlation between the GIV and net export growth is quite stable across various specifications. The first-stage Kleibergen-Paap F-statistic \citep{kleibergen2006generalized}, which is robust to clustered standard errors, is 81.25 in column (4) with all control variables. And the Montiel Olea-Pflueger Efficient F-statistics \citep{olea2013robust} is 82.20 in column (4). Thus, it is very unlikely that our estimates are biased by a weak instrument. 

\comment{We also show an added-variable plot of first-stage regression in figure (\ref{fig:NEP_D92t06_FirstStage}), holding all other variables constant.}

Panel C reports 2SLS estimates. Like OLS and reduced-form estimates, the 2SLS estimates are quite stable as I introduce the baseline controls in columns (2)-(4). As emphasized by \cite{jiang2017have}, it is important to compare the 2SLS estimates with OLS estimates given that 255 papers from the "Big Three" finance journals have the former one as nine times the latter one on average. The key concerns are the bias from a weak IV and publication bias in searching for "blown-up" IV estimates. Besides our two F-statistics, I also confirm that 2SLS estimates are very close to OLS estimates throughout various specifications, where our baseline results in column (4) indicate a ratio of $0.517/0.300=1.723$, much lower than nine. According to column (4), one standard cross-sectional difference in annualized net export growth results in $0.18\% \times 0.517 = 0.093\%$ difference in employment share increase annually, translating into $1.302\%$ difference at the county level from 1992 to 2006. Such an effect is statistically significant at the one percent level. 


\comment{$0.093\%$ cross-sectional difference in annual income growth rate is so small that it is very likely ignored by GSEM policy. }



%------------------------------------------------------------
%\subsection{Net Export and Household Income}
%------------------------------------------------------------
\subsubsection{Net Export and Household Income}

Table (\ref{table:IRSHHIncome.D92t06.4Reg}) reports OLS, reduced-form, second stage, and first stage of the results of household income growth in panels A, B, C, and D. First, panel A column (1) shows the positive and significant impact of net export growth (92-06, annualized) on household income growth (92-06, annualized), without any control. Through columns (2) to (4), the estimates show that the OLS coefficient of the next export growth is almost unaffected by the inclusion of the number of households, household income, and number of housing units in 1992. Panel B reports the reduced-form estimates and shows that gravity-model-based net export growth increases household income growth. This significant impact is quite stable to the inclusion of various controls. 

First-stage estimates in panel D show that the strong positive correlation between the GIV and net export growth is quite stable across various specifications. The first-stage Kleibergen-Paap F-statistic \citep{kleibergen2006generalized}, which is robust to clustered standard errors, is 84.56 in column (4) with all control variables. And the Montiel Olea-Pflueger Efficient F-statistics \citep{olea2013robust} is 86.21 in column (4). Thus, it is very unlikely that our estimates are biased by weak instruments. I also show an added-variable plot of first-stage regression in figure (\ref{fig:NEP_D92t06_FirstStage}), after controlling all other variables.

Panel C reports 2SLS estimates that are quite stable as I introduce the baseline controls in columns (2)-(4). As emphasized by \cite{jiang2017have}, the key concern is that bias from a weak IV is liked to be chosen in a striking direction due to the publication pressure. Besides our two F-statistics, I also confirm that 2SLS estimates are very close to OLS estimates, where our baseline results in column (4) indicate a ratio of $0.695/0.788=0.882$, much lower than nine. Column (4) shows one standard cross-sectional difference in annualized net export growth results in $0.18\% \times 0.695 = 0.12\%$ difference in household income growth, translating into $1.99\%$ difference at the county level from 1992 to 2006. Such an effect is statistically significant at the one percent level. 


\comment{$0.12\%$ cross-sectional difference in annual income growth rate is so small that it is very likely ignored by GSEM policy. }







%------------------------------------------------------------
%\subsection{Net Export and Population}
%------------------------------------------------------------
\subsubsection{Net Export and Population}

Table (\ref{table:WorkAgePop.D92t06.4Reg}) reports OLS, reduced-form, second stage, and first stage of the results of working-age population (age 15-64) growth in panels A, B, C, and D. First, panel A column (1) shows the positive and significant impact of net export growth (92-06, annualized) on working-age population growth (92-06, annualized), without any control. Through columns (2) to (4), the estimates show that the OLS coefficient of the next export growth is almost unaffected by the inclusion of the total population, household income, and number of housing units in 1992. Panel B reports the reduced-form estimates and shows that gravity-model-based net export growth increases household income growth. This significant impact is also quite stable to the inclusion of various controls. 

First-stage estimates in panel D show that the strong positive correlation between the GIV and net export growth is quite stable across various specifications. The first-stage Kleibergen-Paap F-statistic \citep{kleibergen2006generalized}, which is robust to clustered standard errors, is 83.72 in column (4) with all control variables. And the Montiel Olea-Pflueger Efficient F-statistics \citep{olea2013robust} is 85.04 in column (4). Thus, it is very unlikely that our estimates are biased by weak instruments. 

\comment{We also show an added-variable plot of first-stage regression in figure (\ref{fig:NEP_D92t06_FirstStage}), holding all other variables constant.}

Panel C reports 2SLS estimates that are quite unaffected by the inclusion of controls. As emphasized by \cite{jiang2017have}, the key concern is that publication pressure likely picks up a biased but highly significant IV estimate due to a weak instrument. Besides our two F-statistics, I also confirm that 2SLS estimates are very close to OLS estimates, where our baseline results in column (4) indicate a ratio of $0.719/0.985=0.728$, much lower than nine. Column (4) shows one standard cross-sectional difference in annualized net export growth results in $0.18\% \times 0.719 = 0.129\%$ difference in working-age population growth, translating into $2.07\%$ difference at the county level from 1992 to 2006. 


\comment{$0.129\%$ cross-sectional difference in annual working-age population growth rate is so small that it is very likely ignored by GSEM policy. }




%------------------------------------------------------------
% end of the entire section
%------------------------------------------------------------


==> Old/WhyNEP.tex <==
~~

%--------------------------------------------------------------
%--------------------------------------------------------------
% This is the beginning of the entire section of Model
%--------------------------------------------------------------
%--------------------------------------------------------------

%\clearpage
\section{Why Net Export Can Impact Local Economic Conditions}\label{sec:why_NEG}

In the above model, we assume net export growth can increase local employment growth, household income growth, and population growth in the long run. In this section, we first draw insights from regional economics to illustrate why net export growth can be the driving force of the local economy, including the above three elements. Then we explain its feature of geographic variation through insights from economic geography and explain its feature of persistence via insights from international trade. Taken together, from 1992 to 2006, some metropolitan areas benefit from a persistently higher level of net export growth while others suffer from a lower level of net export growth.



\comment{Since private-label mortgages take into consideration of these local economic conditions, creditors understand the higher foreclosure sale prices and higher household income in the HNEG area, given credit expansion in PLM. As a result, PLNJM shows a stronger increase in the HNEG areas.}


\subsection{Insights from Regional Economics}
Regional economic literature defines the economic base as the set of economic activities that a local area provides for the world beyond its boundaries \citep{tiebout1962community, nijkamp1987regional}. This economic base is the most important driving force for local economic growth and hence house prices \citep{nijkamp1987regional,thrall2002business,ling2013real}.\footnote{Some economists criticize that the economic base ignores retirement communities and college towns phenomena.}  The local economic base drives local economic activity and land use through a multiplier process. The economic base activities bring money into the local area, which then is presented and recirculated within the area. The economic base can predict demand-side factors that shape the long-term growth of housing prices, such as employment growth, household income growth, and population growth.\footnote{Section \ref{subsec:NEG_EmpEvi} summarizes the recent empirical evidence.}

Accurate measurement of the composite and growth of the local economic base requires census-style data covering the accounting data of all firms, which is private and impossible to obtain. Alternatively, the County Business Pattern can proxy the composite of the county economic base with manufacturing employment data at the industry level. In addition, the large change in net export growth in manufacturing industries in the U.S. from 1992 to 2006  provides a potential proxy for the growth of the local economic base at the industry level.\footnote{Using the manufacturing sector to proxy the economic base ignores other tradable goods sectors (e.g., food and medical sectors) and the tradable service sector (e.g., medical sector) in the scope of the economic base.} Aggregating the proxies in composite and growth can give us a good measure of the local economic base. To account for the commuting within local areas, we aggregate net export growth at the level of metropolitan areas. The net export growth has enough area coverage (U.S. mainland) and enough time coverage (92-09).



\subsection{Insights from Economic Geography within A Closed Economy}

The feature of geographic variation arises from the fact that the local manufacturing sector tends to cluster within related industries due to internal and external economies of scale. Over time, declining transportation costs and increasing labor mobility have strengthened the pattern of local clusters of related manufacturing industries. 

\comment{
Therefore, some local clusters (metropolitan areas) of labor-intensive manufacturing industries suffer from import growth, while other clusters of high-tech industries benefit from export growth. 

Net export growth can have a huge impact on the above three local economic conditions (employment growth, household income growth, and population growth) in the long run because the local manufacturing sector often clusters within related industries. Such clustering patterns generate a large geographic variation of exposure to international trade since some industries import while others export in significant amounts. Over time, reducing transportation costs and increasing labor mobility both strengthen the geographic variation of exposure to international trade. 
}


The local manufacturing sector tends to cluster within related industries because of internal and external economies of scale. Internal economies of scale arise from the nature of a fixed cost when a larger firm can lower its average cost by increasing quantities of production. Such economies can happen due to a fixed operating cost of a plant, purchasing inputs at volume discounts, and learning in operation \citep{worldbank2009ch4}. The literature documents an increasing trend of corporate concentration due to internal economies of scale. \cite{kwon2022100} study the corporate concentration (e.g., asset share or sales share of top-size business) by digitizing Statistics of Income (SOI) and the associated Corporate Source Book from the Internal Revenue Service (IRS) from 1918 to 2018. They find a persistent increase in the shares accounted for top-size corporations throughout the last century. The rising concentration was stronger for mining and manufacturing industries before the 1970s and stronger for services, retail, and wholesale after the 1970s. Through various tests, they conclude the stronger economies of scale is mostly consistent with the long-run increase in corporate concentration. For a complete survey of empirical literature based on data after the 1980s, see \cite{furman2016benefits} and \cite{pike2018market}.


External economies of scale within an industry arise from the clustering of a larger number of firms, where average cost decreases with the number (or size) of all firms. External economies of scale can work in at least three channels: specialization of suppliers, labor market pooling, and knowledge spillover \citep{krugman2018internationalCh7}. Specialization happens since many manufacturing industries require specialized equipment and support services. A localized industry cluster can provide a large enough market to support a wide range of specialized suppliers so that inputs from suppliers are cheaper than elsewhere \citep{smith17761976}. In addition, a localized industry cluster can create a pooled market for workers and highly specialized skills. This pooled market can reduce the search cost for both firms and workers \citep{marshall1890principles}. Third, a localized industry cluster can create an advantage for local firms in an industry through knowledge spillover, namely an informal exchange of information and ideas at the personal level. This spillover is called the ``Marshall-Arrow-Romer'' (MAR) externality by \cite{glaeser1992growth}. Famous examples include the semiconductor industry concentrated in Silicon Valley, the automobile industry concentrated in Detroit \citep{holmes2004spatial}, and the carpet industry concentrated in Dalton, Georgia \citep{krugman1991increasing}. 

\comment{the financial service industry concentrated in New York, and the entertainment industry concentrated in Hollywood} 

External economies of scale can also attract firms from closely-related industries via the supply chain. First, shoppers (downstream customers) are attracted to places with many sellers for cheaper prices and lower transportation costs. For example, U.S. garment production and distribution were concentrated in New York City shortly after 1900. But many kitting and waving mills moved to North Carolina after World War II to get closer to the supply of yarn and to take advantage of cheaper power, labor, and land \citep{worldbank2009ch4}. Second, outsourcing by the localized industry cluster attracts both the upstream input suppliers and downstream firms since they can profit from productivity gain by specialization \citep{smith17761976}.      

For the above reasons, both internal and external economies of scale can foster a local cluster of several related industries. For a complete survey of the empirical literature on internal and external economies of scale, see \cite{worldbank2009ch4}, and \cite{head2004empirics}. 


Over the last century, declining transportation costs and increasing labor mobility have reinforced the local clusters of related manufacturing industries. The long-term reduction in transportation costs can be seen from the declining share of the transportation section in the US GDP from 8\% in 1929 to 3\% by 1990 \citep{glaeser2004cities}. Over time, the invention of new transportation technology, construction of extensive infrastructure (canal, railroad, and highways), adoption of information technology, and reorganization of logistic methods have all contributed to continuing decline of transportation costs. For a complete review of transportation costs, see \cite{redding2015transportation} and \cite{kim2004historical}. 

Labor mobility in the United States has been steadily increasing from 1900 to 1980 (except for years during the Great Depression and World War II) and only dropped slightly post-1980 \citep{molloy2011internal}. \cite{rosenbloom2004decline} concluded that increased education attainment could largely explain the long-term increase in labor mobility, among other factors. Compared to other developed countries, the United States has the highest labor mobility based on many different measures at different points of time \citep{greenwood1997internal}. Though there is a lack of ideal data for precise comparison among all developed countries across time, researchers have proposed many plausible reasons for the higher labor mobility in the United States relative to Europe: easy availability of housing (larger available land, chapter building cost, less government regulation of housing market), encouraging public policies (on moving towards areas with less population) and long-standing cultural reasons (the United States as ``a nation of immigrants''). For a complete review, see  \cite{molloy2011internal} and \cite{greenwood1997internal}. 


\comment{I shall draw a map to show the geographic variation of net export growth at the metropolitan level
}
%--------------------------------------------------------------
% This is the start of a new subsection. Insights from International Trade in An Open Economy
%--------------------------------------------------------------

\subsection{Insights from International Trade in An Open Economy}


The persistence feature of net export growth at the metropolitan level arises from three dimensions. At the industry level, both comparative advantages across countries and increasing return to scales can make trade patterns persistent over time. At the metropolitan level, clusters of manufacturing industries that rely on low-skill labor or high technology have been established over decades or even more than a century, involving extensive plants built and the migration by workers. Such structure formation is unlikely to change rapidly in a short period of time. Third, at the individual level, human capital accumulation takes both time and investment, making job reallocation across different industries very difficult both locally and remotely. 


In addition, the international trade patterns in the U.S. after World War Two and recent changes since the 1990s highlight the increasing role of trade on local economic growth, especially between 1990 to 2007. From the end of World War Two (WW2) to the 1980s, international trade in the U.S. and other developed countries was dominated by trade between high-income countries (\cite{krugman2008trade}; \cite{worldtradereport2007} ) because (1) high-income countries accounted for most of global GDP and (2) many middle- and low-income countries maintained man-made barriers for trade \citep{hanson2012rise}. For example, world merchandise exports were dominated by developed countries, with 66.4\% in 1948, 72.9\% in 1963, and 68.2\% in 1983 \comment{and 73.3\% in 1993 } \citep[p. 199]{worldtradereport2007}. The percentage for world merchandise imported by developed countries was 66.7\% in 1948, 73.8\% in 1963, and 70.1\% in 1983 \comment{and 72.3\% in 1993} \citep[p. 200]{worldtradereport2007}. In addition, developed countries have been active participants in the General Agreement of Tariffs and Trade (GATT) since 1947, while developing countries were generally not as active till the 1980s \citep{worldtradereport2007}. One important reason was that many developing countries adopted import substitution policies before the 1980s \citep[p. 220]{worldtradereport2007}.


\comment{
Even in 1989, US trade (average of imports and exports) of manufactures with developed countries was almost as twice as the ones from developing countries in 1989 \citep{krugman2008trade}. }


A defining feature of trade between developed countries is that intra-industry trade occupies a larger portion of trade, reflecting product differentiation within industries due to economies of scale and preference for varieties \citep{krugman1979increasing, krugman1980scale}.  For example, the US exports automobiles manufactured by companies such as Chevrolet, Chrysler, Ford, and Tesla, while importing cars from firms such as Honda and Toyota from Japan, BMW and Mercedes Benz from German, and Fiat and Maserati from Italy. For more empirical evidence of the dominant share of intra-industry trade between high-income countries, see \cite{brulhart2008account, coeure2020trade, turkcan2010structure}. This long-term dominance by high-income countries in international trade can foster a long period of within-industry specialization in the U.S. tradable sectors as they can take advantage of economies of scale of global markets. One possible consequence could be an increased size of the local manufacturing clusters relative to the regional economy, resulting in stronger local exposure to trade. 


\comment{ \cite{davis1999economic} provide empirical evidence that economic geography can account for cross-country variation in manufacturing structure, and \cite{davis2003market} provide evidence that economic geography can also explain within-country across-region variation in manufacturing structure. For more empirical evidence of economic geography implied by the new trade theory (that assumes increasing return to scale), see \cite{redding2013economic}.
}


However, between the 1980s and 1990s, many significant changes took place. First, in the 1980s, many developing countries rapidly abolished earlier import substitution strategies and sometimes undertook radical trade liberalizations. Two contributing factors were the wide perception of the limitation of import substitution policies and the success of East Asian regions in international markets \citep[p. 220-221]{worldtradereport2007}. Second, China's economic transition accelerated in the 1990s \citep{amiti2010anatomy}, and India's reforms were initiated in 1991 \citep{rodrik2004hindu}. The result was an immense export supply shock: from 1992 to 2008, the average annual growth in exports was 18 percent in China and 14 percent in India \citep{hanson2012rise}. In addition, North American Free Trade Agreement (NAFTA) in 1994 triggered a significant increase in Mexico's exports to the United States \citep{krugman2008trade} Forth, continuous effects by GATT members resulted in significant tariff reductions by 33 percent between 1980-1987, by 38 percent between 1995-1999 \citep[p. 207]{worldtradereport2007}, and the establishment of the World Trade Organization (WTO) in 1995. Fifth, the Dissolution of the Soviet Union in 1991 triggered many countries in Central and Eastern Europe and the former Soviet Union to apply to accede to the GATT and then the WTO \citep{broadman2006disintegration}. Their trade liberalization increased the whole global market.


All the above forces have contributed to the sharp increase in US imports, particularly with developing countries (with China and Mexico being two leading counties) \citep{krugman2008trade}. For example, the share of US manufacturing imports from low-income countries was 9 percent in 1991, 15 percent in 2000, and eventually 28 percent in 2007 \citep{david2013china}. Such North-South trade is mostly driven by comparative advantages either in productivity differences due to technology or in factor abundance due to natural endowment. Thus the import competition is likely persistent. Meanwhile, US exports had a similar increasing trend: they almost doubled from 1991 to 2007, from less than 600 billion to more than 1 trillion \citep[Figure 1]{feenstra2019us}. The nature of increasing return to scales in many manufacturing industries means that small early advantages could reinforce themselves into substantial superiority over time.  


Consequently, between 1990 to 2007, the US local clusters of labor-intensive manufacturers could potentially suffer heavily from import competition \citep{david2013china}. Meanwhile, local clusters of high-tech manufacturers could potentially benefit from export expansion \citep{feenstra2019us}. In addition, in the era of globalization, the growth of the tradable sector is the engine of economic growth: the growth of world merchandise exports is three times higher than that of world GDP \citep[p. 243]{worldtradereport2007}. Viewed in this vein, features of geographic variation and persistence in net export growth could potentially lead to substantial differences in local economic growth.  



In summary, economic base theory supports that net export growth can be the driving force of the local economy, including growth in employment, household income, and population. Geographic variation due to local clustering of manufacturing and persistence due to trade nature together imply that net export growth can drive the divergence of housing prices in the long term.


\comment{
In summary, the significant surge in US international trade between 1991 and 2007, along with the local clustering of manufacturing, suggests that net export growth may be a driving factor behind disparities in local economic growth.
}

\comment{To sum up, the strong increase in US international trade from 1991 to 2007 and the local clustering of manufacturing potentially mean that trade can cause differences in local economic growth.}

\comment{
In summary, the significant surge in US international trade between 1991 and 2007, along with the local clustering of manufacturing, suggests that trade may be a driving factor behind disparities in local economic growth.
}


\comment{
To measure the impact of trade on a particular industry in manufacturing, net export for each industry shall be used to account for intra-industry trade. Then weighted average net export in a local area is calculated using employment share at the start period as weight. }

\comment{
Counteracting Forces
Even with the above arguments, there are countervailing forces that might reduce or even neutralize the impact of international trade on local economic growth. First, income per capita across US census divisions experienced a persistent long-term trend of convergence between 1900 and 1990 \citep[p. 2992, Figure 3]{kim2004historical}. This empirical fact and the economic forces behind it might reduce or even neutralize the impact of trade on local economic growth across metropolitan areas. Second, industry (especially manufacturing) concentration across US census divisions experienced a long trend of decline in the twentieth century \citep{kim1995expansion, crafts2021spatial}. This declining concentration of manufacturing industries might be strong enough to buffer the rising impact of US imports and exports. Third, the strong growth of the service sector (especially low-skilled service occupants) from 1990 to 2007 \citep{acemoglu2011skills} might absorb much of the effect of net export growth. On the one hand, the import-induced unemployed labor force can be primarily reallocated into retail and service industries locally. On the other hand, the export-induced employment growth may not be large enough since the overall employment growth can be dominated by retail and service industries locally. 
}



\subsection{Empirical Evidence}\label{subsec:NEG_EmpEvi}
In the literature, searchers show evidence of local employment changes due to imports \citep{autor2013china, pierce2016surprisingly} and exports \citep{feenstra2005world}. The literature also documents the local household income changes due to imports \citep{barrot2022import} and exports \cite{minot1998export}. For changes in population growth (including migration), \cite{greenland2019import} provide causal evidence on imports, and \cite{li2023globalization} provide causal evidence on exports. 

We are the first to combine export and import as net export and examine its impact on the three above local economic conditions. This step is necessary for several reasons. First, imports and exports can be both in large amounts in a single industry like the U.S. auto industry since they can reflect within-industry horizontal specialization. Our net export growth measure can sum up both effects within the same industry. Second, a local area can be exposed to both imports and exports so that the two effects may be completely offset. Our net export growth measure thus can sum both effects at the local level. Third, the pieces of evidence from the above literature may not all cover exactly the same period in the United States. 

In the empirical tests in Section \ref{subsec:NEG_LocalEconConditions}, we verify that net export growth cause a differential higher increase in local employment growth, household income growth, and population growth in the HNEG areas. Please note that we do not claim such verification as our contribution. 



%--------------------------------------------------------------
%--------------------------------------------------------------
% This is the end of the entire section 
%--------------------------------------------------------------
%--------------------------------------------------------------


==> Table/table_GSEM.D99t05vsD05t08.2SLS.tex <==
%----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_GSEM.D99t05vsD05t08.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of GSEM Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{99,05} \&  \triangle_{05,08}  Ln(GSEM_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(GSEM_{c})$ is the stacked growth rate of the dollar amount of government-sponsored enterprise mortgages (GSEMs) at county $c$ 99-05 and 05-08. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m} $ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{99,05} $ and $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{05,08} $ as IVs for $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{99,05}$ and $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{05,08}$. Each regression is weighted by the natural logarithm of housing units in the start year 1999. For the first-stage F-test of two non-stack samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. We report Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_GSEM.D99t05vsD05t08.2SLS}


\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{GSEM Growth (99-05 and 05-08, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum99t05&    1.889   &    4.626** &    3.071   &    3.149   &    2.205   \\
               &  (2.539)   &  (2.265)   &  (2.329)   &  (2.307)   &  (2.470)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&   -3.514   &   -6.394   &   -7.124   &   -4.614   &   -5.817   \\
               &  (4.956)   &  (4.648)   &  (5.245)   &  (5.172)   &  (5.181)   \\
\addlinespace
Dummry 99-05   &    0.046***&    1.074***&    0.851***&    1.216***&    1.289***\\
               &  (0.008)   &  (0.187)   &  (0.207)   &  (0.329)   &  (0.339)   \\
\addlinespace
Dummry 05-08   &   -0.080***&   -1.479** &   -1.677***&   -0.456   &   -0.133   \\
               &  (0.017)   &  (0.622)   &  (0.606)   &  (0.688)   &  (0.666)   \\
\addlinespace
Ln(Num of HH, 99) x pd\_D99t05&            &   -0.015***&    0.011   &    0.054   &    0.047   \\
               &            &  (0.002)   &  (0.036)   &  (0.034)   &  (0.032)   \\
\addlinespace
Ln(Num of HH, 99) x pd\_D05t08&            &    0.014** &    0.020   &   -0.068   &   -0.074   \\
               &            &  (0.006)   &  (0.088)   &  (0.084)   &  (0.082)   \\
\addlinespace
Ln(HH Income, 99) x pd\_D99t05&            &   -0.067***&   -0.049** &   -0.090***&   -0.097***\\
               &            &  (0.020)   &  (0.023)   &  (0.033)   &  (0.033)   \\
\addlinespace
Ln(HH Income, 99) x pd\_D05t08&            &    0.121*  &    0.167** &    0.071   &    0.046   \\
               &            &  (0.066)   &  (0.069)   &  (0.074)   &  (0.070)   \\
\addlinespace
Ratio of Labor Force (1999) x pd\_D99t05&            &   -0.214***&   -0.228** &   -0.327***&   -0.334***\\
               &            &  (0.075)   &  (0.091)   &  (0.084)   &  (0.089)   \\
\addlinespace
Ratio of Labor Force (1999) x pd\_D05t08&            &   -0.090   &   -0.281   &   -0.094   &   -0.189   \\
               &            &  (0.199)   &  (0.218)   &  (0.198)   &  (0.212)   \\
\addlinespace
Ln(Num of HU, 99) x pd\_D99t05&            &            &   -0.023   &   -0.065*  &   -0.059*  \\
               &            &            &  (0.037)   &  (0.035)   &  (0.033)   \\
\addlinespace
Ln(Num of HU, 99) x pd\_D05t08&            &            &   -0.036   &    0.040   &    0.041   \\
               &            &            &  (0.088)   &  (0.085)   &  (0.083)   \\
\addlinespace
Housing supply elasticity x pd\_D99t05&            &            &    0.002   &    0.002   &    0.002   \\
               &            &            &  (0.003)   &  (0.003)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x pd\_D05t08&            &            &   -0.005   &   -0.002   &   -0.003   \\
               &            &            &  (0.006)   &  (0.005)   &  (0.005)   \\
\addlinespace
House Vacancy Rate (1999) x pd\_D99t05&            &            &    0.216** &    0.247***&    0.232** \\
               &            &            &  (0.093)   &  (0.094)   &  (0.096)   \\
\addlinespace
House Vacancy Rate (1999) x pd\_D05t08&            &            &   -0.145   &   -0.276*  &   -0.226   \\
               &            &            &  (0.138)   &  (0.144)   &  (0.144)   \\
\addlinespace
Ratio of Renters (1999) x pd\_D99t05&            &            &   -0.032   &    0.045   &   -0.012   \\
               &            &            &  (0.061)   &  (0.061)   &  (0.065)   \\
\addlinespace
Ratio of Renters (1999) x pd\_D05t08&            &            &    0.586***&    0.159   &    0.311** \\
               &            &            &  (0.145)   &  (0.104)   &  (0.140)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D99t05&            &            &            &    0.172** &    0.066   \\
               &            &            &            &  (0.083)   &  (0.096)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D05t08&            &            &            &    0.147   &    0.126   \\
               &            &            &            &  (0.153)   &  (0.163)   \\
\addlinespace
Ratio of White Race (1999) x pd\_D99t05&            &            &            &    0.085***&    0.063** \\
               &            &            &            &  (0.024)   &  (0.024)   \\
\addlinespace
Ratio of White Race (1999) x pd\_D05t08&            &            &            &   -0.145***&   -0.098** \\
               &            &            &            &  (0.048)   &  (0.048)   \\
\addlinespace
Ratio of Immigration (90-00) x pd\_D99t05&            &            &            &   -0.326   &   -0.230   \\
               &            &            &            &  (0.202)   &  (0.196)   \\
\addlinespace
Ratio of Immigration (90-00) x pd\_D05t08&            &            &            &    1.767***&    1.483***\\
               &            &            &            &  (0.477)   &  (0.472)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x pd\_D99t05&            &            &            &            &    1.176***\\
               &            &            &            &            &  (0.356)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x pd\_D05t08&            &            &            &            &   -1.751** \\
               &            &            &            &            &  (0.782)   \\
\addlinespace
Ratio of Health Emp (1999) x pd\_D99t05&            &            &            &            &    0.733** \\
               &            &            &            &            &  (0.294)   \\
\addlinespace
Ratio of Health Emp (1999) x pd\_D05t08&            &            &            &            &   -0.879   \\
               &            &            &            &            &  (0.558)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x pd\_D99t05&            &            &            &            &    0.305   \\
               &            &            &            &            &  (0.339)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x pd\_D05t08&            &            &            &            &    0.940   \\
               &            &            &            &            &  (0.723)   \\
\addlinespace
Ratio of College Students (1999) x pd\_D99t05&            &            &            &            &    0.130   \\
               &            &            &            &            &  (0.133)   \\
\addlinespace
Ratio of College Students (1999) x pd\_D05t08&            &            &            &            &   -0.856** \\
               &            &            &            &            &  (0.342)   \\
\midrule
Obs            &     1584   &     1584   &     1402   &     1402   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, Non-stack Sample)  &    23.36   &    23.11   &    16.44   &    17.78   &    17.75   \\
MOP F-Eff (99-05, Non-stack Sample) &    22.91   &    22.63   &    16.08   &    17.44   &    17.40   \\
CoefEqual\_Chi2 &    0.727   &    3.639   &    2.404   &    1.380   &    1.479   \\
CoefEqual\_PValue &    0.394   &    0.056   &    0.121   &    0.240   &    0.224   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_GSEM.D99t05vsD05t08.2SLS.wide.tex <==
%----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_GSEM.D99t05vsD05t08.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of GSEM Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{99,05} \&  \triangle_{05,08}  Ln(GSEM_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(GSEM_{c})$ is the stacked growth rate of the dollar amount of government-sponsored enterprise mortgages (GSEMs) at county $c$ 99-05 and 05-08. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m} $ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{99,05} $ and $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{05,08} $ as IVs for $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{99,05}$ and $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{05,08}$. Each regression is weighted by the natural logarithm of housing units in the start year 1999. For the first-stage F-test of two non-stack samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. We report Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_GSEM.D99t05vsD05t08.2SLS.wide}


\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{10}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{10}{c}{GSEM Growth (99-05 and 05-08, annualized)} \\
            \cmidrule{2-11} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}&\multicolumn{2}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum99t05&    1.889   &  (2.539)&    4.626** &  (2.265)&    3.071   &  (2.329)&    3.149   &  (2.307)&    2.205   &  (2.470)\\ 
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&   -3.514   &  (4.956)&   -6.394   &  (4.648)&   -7.124   &  (5.245)&   -4.614   &  (5.172)&   -5.817   &  (5.181)\\ 
\addlinespace
Dummry 99-05   &    0.046***&  (0.008)&    1.074***&  (0.187)&    0.851***&  (0.207)&    1.216***&  (0.329)&    1.289***&  (0.339)\\ 
\addlinespace
Dummry 05-08   &   -0.080***&  (0.017)&   -1.479** &  (0.622)&   -1.677***&  (0.606)&   -0.456   &  (0.688)&   -0.133   &  (0.666)\\ 
\addlinespace
Ln(Num of HH, 99) x pd\_D99t05&            &         &   -0.015***&  (0.002)&    0.011   &  (0.036)&    0.054   &  (0.034)&    0.047   &  (0.032)\\ 
\addlinespace
Ln(Num of HH, 99) x pd\_D05t08&            &         &    0.014** &  (0.006)&    0.020   &  (0.088)&   -0.068   &  (0.084)&   -0.074   &  (0.082)\\ 
\addlinespace
Ln(HH Income, 99) x pd\_D99t05&            &         &   -0.067***&  (0.020)&   -0.049** &  (0.023)&   -0.090***&  (0.033)&   -0.097***&  (0.033)\\ 
\addlinespace
Ln(HH Income, 99) x pd\_D05t08&            &         &    0.121*  &  (0.066)&    0.167** &  (0.069)&    0.071   &  (0.074)&    0.046   &  (0.070)\\ 
\addlinespace
Ratio of Labor Force (1999) x pd\_D99t05&            &         &   -0.214***&  (0.075)&   -0.228** &  (0.091)&   -0.327***&  (0.084)&   -0.334***&  (0.089)\\ 
\addlinespace
Ratio of Labor Force (1999) x pd\_D05t08&            &         &   -0.090   &  (0.199)&   -0.281   &  (0.218)&   -0.094   &  (0.198)&   -0.189   &  (0.212)\\ 
\addlinespace
Ln(Num of HU, 99) x pd\_D99t05&            &         &            &         &   -0.023   &  (0.037)&   -0.065*  &  (0.035)&   -0.059*  &  (0.033)\\ 
\addlinespace
Ln(Num of HU, 99) x pd\_D05t08&            &         &            &         &   -0.036   &  (0.088)&    0.040   &  (0.085)&    0.041   &  (0.083)\\ 
\addlinespace
Housing supply elasticity x pd\_D99t05&            &         &            &         &    0.002   &  (0.003)&    0.002   &  (0.003)&    0.002   &  (0.003)\\ 
\addlinespace
Housing supply elasticity x pd\_D05t08&            &         &            &         &   -0.005   &  (0.006)&   -0.002   &  (0.005)&   -0.003   &  (0.005)\\ 
\addlinespace
House Vacancy Rate (1999) x pd\_D99t05&            &         &            &         &    0.216** &  (0.093)&    0.247***&  (0.094)&    0.232** &  (0.096)\\ 
\addlinespace 
House Vacancy Rate (1999) x pd\_D05t08&            &         &            &         &   -0.145   &  (0.138)&   -0.276*  &  (0.144)&   -0.226   &  (0.144)\\\addlinespace
Ratio of Renters (1999) x pd\_D99t05&            &         &            &         &   -0.032   &  (0.061)&    0.045   &  (0.061)&   -0.012   &  (0.065)\\ 
\addlinespace
Ratio of Renters (1999) x pd\_D05t08&            &         &            &         &    0.586***&  (0.145)&    0.159   &  (0.104)&    0.311** &  (0.140)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D99t05&            &         &            &         &            &         &    0.172** &  (0.083)&    0.066   &  (0.096)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D05t08&            &         &            &         &            &         &    0.147   &  (0.153)&    0.126   &  (0.163)\\ 
\addlinespace
Ratio of White Race (1999) x pd\_D99t05&            &         &            &         &            &         &    0.085***&  (0.024)&    0.063** &  (0.024)\\ 
\addlinespace
Ratio of White Race (1999) x pd\_D05t08&            &         &            &         &            &         &   -0.145***&  (0.048)&   -0.098** &  (0.048)\\ 
\addlinespace
Ratio of Immigration (90-00) x pd\_D99t05&            &         &            &         &            &         &   -0.326   &  (0.202)&   -0.230   &  (0.196)\\ 
\addlinespace
Ratio of Immigration (90-00) x pd\_D05t08&            &         &            &         &            &         &    1.767***&  (0.477)&    1.483***&  (0.472)\\ 
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x pd\_D99t05&            &         &            &         &            &         &            &         &    1.176***&  (0.356)\\ 
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x pd\_D05t08&            &         &            &         &            &         &            &         &   -1.751** &  (0.782)\\ 
\addlinespace
Ratio of Health Emp (1999) x pd\_D99t05&            &         &            &         &            &         &            &         &    0.733** &  (0.294)\\ 
\addlinespace
Ratio of Health Emp (1999) x pd\_D05t08&            &         &            &         &            &         &            &         &   -0.879   &  (0.558)\\ 
\addlinespace
Ratio of Tradable Service Emp (1999) x pd\_D99t05&            &         &            &         &            &         &            &         &    0.305   &  (0.339)\\ 
\addlinespace
Ratio of Tradable Service Emp (1999) x pd\_D05t08&            &         &            &         &            &         &            &         &    0.940   &  (0.723)\\ 
\addlinespace
Ratio of College Students (1999) x pd\_D99t05&            &         &            &         &            &         &            &         &    0.130   &  (0.133)\\ 
\addlinespace
Ratio of College Students (1999) x pd\_D05t08&            &         &            &         &            &         &            &         &   -0.856** &  (0.342)\\ 
\addlinespace
\midrule
Obs            &     1584   &         &     1584   &         &     1402   &         &     1402   &         &     1402   &         \\
Cluster SE     &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat      &    23.36   &         &    23.11   &         &    16.44   &         &    17.78   &         &    17.75   &         \\
MOP F-Eff      &    22.91   &         &    22.63   &         &    16.08   &         &    17.44   &         &    17.40   &         \\
CoefEqual\_Chi2 &    0.727   &         &    3.639   &         &    2.404   &         &    1.380   &         &    1.479   &         \\
CoefEqual\_PValue &    0.394   &         &    0.056   &         &    0.121   &         &    0.240   &         &    0.224   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_GSEM.D99t05vsD05t08.4Reg.tex <==



%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_GSEM.D99t05vsD05t08.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Stacked Regressions of GSEM Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports OLS, reduced-form, first stage and second stages of 2SLS stacked regression $\triangle_{99,05} \&  \triangle_{05,08}  Ln(GSEM_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(GSEM_{c})$ is the stacked growth rate of the dollar amount of government-sponsored enterprise mortgages (GSEMs) at county $c$ 99-05 and 05-08. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m} $ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{99,05} $ and $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{05,08} $ as IVs for $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{99,05}$ and $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{05,08}$. Each regression is weighted by the natural logarithm of housing units in the start year 1999. For the first-stage F-test of two non-stack samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_GSEM.D99t05vsD05t08.4Reg}

\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
Dep Var (Panel A, B, and C)                      &\multicolumn{5}{c}{GSEM Growth (99-05 \& 05-08, annualized)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\     


\midrule
\multicolumn{6}{l}{\textbf{Panel A. OLS estimates}} \\
Net Export Growth (99-05, An) x Dum99t05&    2.928** &    4.552***&    3.800***&    3.286** &    2.850** \\
               &  (1.360)   &  (1.380)   &  (1.368)   &  (1.338)   &  (1.308)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&    1.237   &   -0.598   &   -2.144   &   -1.402   &   -2.751   \\
               &  (3.075)   &  (2.779)   &  (2.853)   &  (2.922)   &  (2.848)   \\
\addlinespace
R2-adj         &    0.224   &    0.298   &    0.374   &    0.436   &    0.453   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel B. Reduced-form estimates}} \\
GIV Net Export Growth (99-05, An) x Dum99t05&    2.173   &    5.288** &    3.373   &    3.522   &    2.350   \\
               &  (2.987)   &  (2.567)   &  (2.633)   &  (2.515)   &  (2.673)   \\
\addlinespace
GIV Net Export Growth (99-05, An) x Dum05t08&   -4.043   &   -7.309   &   -7.825   &   -5.160   &   -6.201   \\
               &  (5.671)   &  (5.218)   &  (5.700)   &  (5.680)   &  (5.510)   \\
\addlinespace
R2-adj         &    0.224   &    0.298   &    0.374   &    0.436   &    0.453   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An) x Dum99t05&    1.889   &    4.626** &    3.071   &    3.149   &    2.205   \\
               &  (2.539)   &  (2.265)   &  (2.329)   &  (2.307)   &  (2.470)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&   -3.514   &   -6.394   &   -7.124   &   -4.614   &   -5.817   \\
               &  (4.956)   &  (4.648)   &  (5.245)   &  (5.172)   &  (5.181)   \\
\addlinespace
\addlinespace


Dep Var (Panel D): &\multicolumn{5}{c}{Net Export Growth (99-05, An)} \\ 
\midrule 
\multicolumn{6}{l}{\textbf{Panel D . First-stage estimates only for 99-05 (non-stack sample)}} \\
\addlinespace
GIV Net Export Growth (99-05, An) x Dum99t05&    1.150***&    1.143***&    1.098***&    1.118***&    1.105***\\
               &  (0.238)   &  (0.238)   &  (0.271)   &  (0.265)   &  (0.262)   \\
\addlinespace
KP F-Stat      &    23.36   &    23.11   &    16.44   &    17.78   &    17.75   \\
MOP F-Eff &    22.91   &    22.63   &    16.08   &    17.44   &    17.40   \\

\addlinespace
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Controls (for all Panels)}} \\
DumPeriod &            &  Y   &   Y    & Y    &  Y    \\
Basic Controls x DumPeriod &            &  Y   &   Y    & Y    &  Y    \\
Housing Controls x DumPeriod &           &      & Y       & Y    &  Y    \\
Demographic Controls x DumPeriod &            &      &        &  Y    &  Y    \\
Industry Controls x DumPeriod &            &      &        &      &  Y    \\
\midrule              
Obs (Panel A, B, and C)          &     1584   &     1584   &     1402   &     1402   &     1402   \\
Obs (Panel D)           &      792   &      792   &      701   &      701   &      701   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   &Ln(HU99)   &Ln(HU99)   &Ln(HU99)    \\
\bottomrule
\end{tabular}

} % end of resize box

\end{table}


==> Table/table_GSEMvsPLNJM.D99t05.2SLS.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_GSEMvsPLNJM.D99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of GSEM and PLNJM Growth in Boom Period (99-05) on Net Export Growth (99-05)} \smallskip \newline
{\footnotesize
This table reports 2SLS stacked regression $\triangle_{99,05} Ln(GSEMnPLNJM_{c}) = \beta_{G} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{G} + \beta_{P} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{P} + \gamma_{G}* \bm{Controls_{c}} \times Dum_{G} + \gamma_{P}* \bm{Controls_{c}} \times Dum_{P}  + \alpha_{G} + \alpha_{P} + \epsilon_{G, c} + \epsilon_{P, c}$. The left-hand-side dependent variable $\triangle_{99,05} Ln(GSEMnPLNJM_{c})$ is the stacked growth rate of the dollar amount of either government-sponsored enterprise mortgages (GSEM) or private-label (non-jumbo) mortgages (PLNJM) at county $c$ 99-05. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in 1999. We use the gravity model-based instrumental variable ($\triangle_{99,05}\text{givNetExp}_{m}$) as IV for $\triangle_{99,05}\text{NetExp}_{m}$. For the first-stage F-test, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Regression is weighted by the natural logarithm of housing units in 1999. We report the statistics and p-values for the tests of coefficient equality between $\beta_{G}$ and $\beta_{P}$. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
\smallskip
} % end of caption
\label{table_GSEMvsPLNJM.D99t05.2SLS}

\vspace{-2mm}

\resizebox{0.54\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{GSEM and PLNJM Growth (1999-2005, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum\_GSEM&    1.889   &    4.626** &    3.071   &    3.149   &    2.205   \\
               &  (2.539)   &  (2.265)   &  (2.329)   &  (2.307)   &  (2.470)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum\_PLNJM&   13.694***&   13.365***&   11.145***&   10.851***&   10.992***\\
               &  (3.547)   &  (3.643)   &  (3.254)   &  (3.331)   &  (3.231)   \\
\addlinespace
Dum\_GSEM       &    0.046***&    1.074***&    0.851***&    1.216***&    1.289***\\
               &  (0.008)   &  (0.187)   &  (0.207)   &  (0.329)   &  (0.339)   \\
\addlinespace
Dum\_PLNJM      &    0.200***&    0.181   &    0.352   &   -0.339   &   -0.446   \\
               &  (0.009)   &  (0.212)   &  (0.236)   &  (0.371)   &  (0.358)   \\
\addlinespace
Ln(Num of HH, 99) x Dum\_GSEM&            &   -0.015***&    0.011   &    0.054   &    0.047   \\
               &            &  (0.002)   &  (0.036)   &  (0.034)   &  (0.032)   \\
\addlinespace
Ln(Num of HH, 99) x Dum\_PLNJM&            &    0.006** &    0.021   &    0.003   &   -0.007   \\
               &            &  (0.003)   &  (0.032)   &  (0.031)   &  (0.031)   \\
\addlinespace
Ln(HH Income, 99) x Dum\_GSEM&            &   -0.067***&   -0.049** &   -0.090***&   -0.097***\\
               &            &  (0.020)   &  (0.023)   &  (0.033)   &  (0.033)   \\
\addlinespace
Ln(HH Income, 99) x Dum\_PLNJM&            &   -0.004   &   -0.027   &    0.035   &    0.043   \\
               &            &  (0.022)   &  (0.025)   &  (0.036)   &  (0.034)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum\_GSEM&            &   -0.214***&   -0.228** &   -0.327***&   -0.334***\\
               &            &  (0.075)   &  (0.091)   &  (0.084)   &  (0.089)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum\_PLNJM&            &   -0.021   &    0.081   &    0.127   &    0.165   \\
               &            &  (0.107)   &  (0.099)   &  (0.102)   &  (0.102)   \\
\addlinespace
Ln(Num of HU, 99) x Dum\_GSEM&            &            &   -0.023   &   -0.065*  &   -0.059*  \\
               &            &            &  (0.037)   &  (0.035)   &  (0.033)   \\
\addlinespace
Ln(Num of HU, 99) x Dum\_PLNJM&            &            &   -0.010   &    0.009   &    0.021   \\
               &            &            &  (0.033)   &  (0.032)   &  (0.032)   \\
\addlinespace
Housing supply elasticity x Dum\_GSEM&            &            &    0.002   &    0.002   &    0.002   \\
               &            &            &  (0.003)   &  (0.003)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x Dum\_PLNJM&            &            &   -0.011***&   -0.011***&   -0.010***\\
               &            &            &  (0.003)   &  (0.003)   &  (0.003)   \\
\addlinespace
House Vacancy Rate (1999) x Dum\_GSEM&            &            &    0.216** &    0.247***&    0.232** \\
               &            &            &  (0.093)   &  (0.094)   &  (0.096)   \\
\addlinespace
House Vacancy Rate (1999) x Dum\_PLNJM&            &            &    0.179** &    0.187** &    0.106   \\
               &            &            &  (0.087)   &  (0.084)   &  (0.084)   \\
\addlinespace
Ratio of Renters (1999) x Dum\_GSEM&            &            &   -0.032   &    0.045   &   -0.012   \\
               &            &            &  (0.061)   &  (0.061)   &  (0.065)   \\
\addlinespace
Ratio of Renters (1999) x Dum\_PLNJM&            &            &   -0.107** &   -0.054   &   -0.113*  \\
               &            &            &  (0.053)   &  (0.058)   &  (0.058)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum\_GSEM&            &            &            &    0.172** &    0.066   \\
               &            &            &            &  (0.083)   &  (0.096)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum\_PLNJM&            &            &            &   -0.239** &   -0.176   \\
               &            &            &            &  (0.094)   &  (0.108)   \\
\addlinespace
Ratio of White Race (1999) x Dum\_GSEM&            &            &            &    0.085***&    0.063** \\
               &            &            &            &  (0.024)   &  (0.024)   \\
\addlinespace
Ratio of White Race (1999) x Dum\_PLNJM&            &            &            &    0.018   &    0.000   \\
               &            &            &            &  (0.035)   &  (0.034)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum\_GSEM&            &            &            &   -0.326   &   -0.230   \\
               &            &            &            &  (0.202)   &  (0.196)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum\_PLNJM&            &            &            &    0.138   &    0.250   \\
               &            &            &            &  (0.197)   &  (0.200)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x Dum\_GSEM&            &            &            &            &    1.176***\\
               &            &            &            &            &  (0.356)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x Dum\_PLNJM&            &            &            &            &    1.726***\\
               &            &            &            &            &  (0.631)   \\
\addlinespace
Ratio of Health Emp (1999) x Dum\_GSEM&            &            &            &            &    0.733** \\
               &            &            &            &            &  (0.294)   \\
\addlinespace
Ratio of Health Emp (1999) x Dum\_PLNJM&            &            &            &            &    0.410   \\
               &            &            &            &            &  (0.410)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x Dum\_GSEM&            &            &            &            &    0.305   \\
               &            &            &            &            &  (0.339)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x Dum\_PLNJM&            &            &            &            &   -0.582*  \\
               &            &            &            &            &  (0.327)   \\
\addlinespace
Ratio of College Students (1999) x Dum\_GSEM&            &            &            &            &    0.130   \\
               &            &            &            &            &  (0.133)   \\
\addlinespace
Ratio of College Students (1999) x Dum\_PLNJM&            &            &            &            &    0.103   \\
               &            &            &            &            &  (0.142)   \\
\midrule
Obs            &     1584   &     1584   &     1402   &     1402   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (Non-Stack Sample)     &    23.36   &    23.11   &    16.44   &    17.78   &    17.11   \\
MOP F-Stat (Non-Stack Sample) &    22.91   &    22.63   &    16.08   &    17.44   &    16.83   \\
CoefEqual\_Chi2 &    8.165   &    7.083   &    6.247   &    6.022   &    6.646   \\
CoefEqual\_PValue&    0.004   &    0.008   &    0.012   &    0.014   &    0.010   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_HPI.D91t19.NEG.D91t07.2SLS_HousingRegulation.tex <==
%-----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D91t19.NEG.D91t07.2SLS_HousingRegulation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Regression of House Price Growth (91-19) on Net Export Growth (91-07)} \smallskip \newline
{\footnotesize 
This table reports 2SLS regression $\triangle_{91,19} Ln(HPI_{c}) = \beta * \triangle_{91,07} \text{NetExp}_{m} + \gamma* \bm{Controls_{c}} + \alpha + \epsilon_{c}$. The left-hand-side dependent variable $\triangle_{91,19} Ln(HPI_{c})$ is the growth rate of the house price index at county $c$ 91-19, and the key variable of interest $\triangle_{91,07} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA09 code) $m$ 91-07. $Controls_{c}$ indicates control variables at county $c$ in 1991. We use the gravity model-based instrumental variable ($\triangle_{91,07}\text{givNetExp}_{m}$) as IV for $\triangle_{91,07}\text{NetExp}_{m}$. For the first-stage F-test, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Regression is weighted by the natural logarithm of housing units in 1991. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
\smallskip \newline
} % end of caption
\label{table_HPI.D91t19.NEG.D91t07.2SLS_HousingRegulation}

\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{5}{c}}
\toprule
            &\multicolumn{5}{c}{House Price Growth (1991-2019, 07USD, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (91-07, An, 07USD)&    0.762***&    0.594*  &    0.539*  &    0.747** &    0.536   \\
               &  (0.218)   &  (0.305)   &  (0.320)   &  (0.291)   &  (0.327)   \\
\addlinespace
Ln(Num of HH, 1991)&   -0.011***&   -0.015***&   -0.017***&   -0.014***&   -0.017***\\
               &  (0.004)   &  (0.005)   &  (0.005)   &  (0.005)   &  (0.005)   \\
\addlinespace
Ln(HH Income, 1991)&   -0.009***&   -0.014***&   -0.015***&   -0.012***&   -0.015***\\
               &  (0.003)   &  (0.004)   &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ratio of Labor Force (1989)&    0.029***&    0.046***&    0.039***&    0.028***&    0.044***\\
               &  (0.009)   &  (0.011)   &  (0.010)   &  (0.010)   &  (0.010)   \\
\addlinespace
Ratio of Bachelor Educated (1989)&    0.023***&    0.027***&    0.030***&    0.025***&    0.029***\\
               &  (0.006)   &  (0.007)   &  (0.007)   &  (0.007)   &  (0.006)   \\
\addlinespace
Ratio of White Race (1989)&    0.010***&    0.008** &    0.009***&    0.009***&    0.008** \\
               &  (0.003)   &  (0.003)   &  (0.003)   &  (0.003)   &  (0.003)   \\
\addlinespace
Ratio of Immigration (80-90)&    0.118***&    0.109***&    0.109***&    0.114***&    0.102***\\
               &  (0.016)   &  (0.017)   &  (0.018)   &  (0.018)   &  (0.017)   \\
\addlinespace
Ratio of Age 65 Above (1989)&    0.017*  &    0.017   &    0.019*  &    0.009   &    0.017   \\
               &  (0.010)   &  (0.011)   &  (0.012)   &  (0.013)   &  (0.011)   \\
\addlinespace
Ln(Num of HU, 1991)&    0.011***&    0.015***&    0.016***&    0.013***&    0.016***\\
               &  (0.004)   &  (0.005)   &  (0.005)   &  (0.005)   &  (0.005)   \\
\addlinespace
House Vacancy Rate (1989)&    0.013   &    0.005   &    0.005   &    0.009   &    0.001   \\
               &  (0.008)   &  (0.010)   &  (0.009)   &  (0.009)   &  (0.010)   \\
\addlinespace
Ratio of Renters (1989)&    0.005   &    0.008   &    0.010*  &    0.008   &    0.008*  \\
               &  (0.005)   &  (0.005)   &  (0.005)   &  (0.005)   &  (0.005)   \\
\addlinespace
Share of Undevelopable Land (50km Radius)&            &    0.010***&            &            &    0.007***\\
               &            &  (0.002)   &            &            &  (0.003)   \\
\addlinespace
Housing supply elasticity&            &            &   -0.002***&            &   -0.001*  \\
               &            &            &  (0.000)   &            &  (0.000)   \\
\addlinespace
Wharton Regulation Index&            &            &            &    0.002***&    0.001   \\
               &            &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Constant       &    0.077** &    0.110***&    0.134***&    0.104***&    0.131***\\
               &  (0.032)   &  (0.034)   &  (0.034)   &  (0.036)   &  (0.034)   \\

\midrule
Obs           &      877   &      740   &      740   &      740   &      740   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU91)   & Ln(HU91)   & Ln(HU91)   & Ln(HU91)   & Ln(HU91)   \\
KP F-Stat      &    81.72   &    58.84   &    58.42   &    58.66   &    57.48   \\
MOP F-Stat     &    81.72   &    58.84   &    58.42   &    58.66   &    57.48   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table/table_HPI.D91t99vsD99t05.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D91t99vsD99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of House Price Growth on Net Export Growth in Prior (91-99) and Boom (99-05) Periods } \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{91,99} \& \triangle_{99,05} Ln(HPI_{c}) = \beta_{91,99} * \triangle_{91,99} \text{NetExp}_{m} \times Dum_{91,99} + \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \gamma_{91,99}* \bm{Controls_{c}} \times Dum_{91,99} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05}  + \alpha_{91,99} + \alpha_{99,05} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{91,99} \& \triangle_{99,05} Ln(HPI_{c})$ is the stacked growth rate of house price index at county $c$ 91-99 and 99-05. The key variable of interest $\triangle_{91,99} \text{NetExp}_{m}$ and $\triangle_{99,05} \text{NetExp}_{m}$ are the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 91-99 and 99-05, respectively. $Controls_{c}$ indicates control variables at county $c$ in the period start year either 1991 or 1999. We use the gravity model-based instrumental variable $\triangle_{91,99}\text{givNetExp}_{m}$ and $\triangle_{99,05}\text{givNetExp}_{m}$ as IVs for $\triangle_{91,99}\text{NetExp}_{m}$ and $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in start year (either 1991 or 1999). We report the statistics and p-values for the tests of coefficient equality between $\beta_{91,99}$ and $\beta_{99,05}$. For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. We report Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_HPI.D91t99vsD99t05.2SLS}

\vspace{-2mm}

\resizebox{0.56\columnwidth}{!}{%


\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{House Price Growth (07USD, 91-99 \& 99-05, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (91-99, An) x Dum91t99&   -3.530** &   -3.125*  &   -2.037   &   -1.736   &   -1.902   \\
               &  (1.684)   &  (1.687)   &  (1.719)   &  (1.743)   &  (1.767)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum99t05&    6.926***&    6.020***&    4.470***&    4.976***&    4.884***\\
               &  (2.327)   &  (2.316)   &  (1.725)   &  (1.805)   &  (1.780)   \\
\addlinespace
Dum91t99   &    0.007** &    0.183***&    0.181***&    0.286***&    0.323***\\
               &  (0.003)   &  (0.046)   &  (0.049)   &  (0.081)   &  (0.095)   \\
\addlinespace
Dum99t05   &    0.055***&   -0.478***&   -0.429***&   -0.464***&   -0.502***\\
               &  (0.006)   &  (0.081)   &  (0.079)   &  (0.131)   &  (0.128)   \\
\addlinespace
Ln(Num of HH, 91) x Dum91t99&            &   -0.002***&   -0.043***&   -0.034***&   -0.031***\\
               &            &  (0.001)   &  (0.011)   &  (0.010)   &  (0.010)   \\
\addlinespace
Ln(Num of HH, 99) x Dum99t05&            &    0.007***&    0.031** &    0.014   &    0.008   \\
               &            &  (0.002)   &  (0.014)   &  (0.013)   &  (0.013)   \\
\addlinespace
Ln(HH Income, 91) x Dum91t99&            &   -0.017***&   -0.018***&   -0.030***&   -0.032***\\
               &            &  (0.005)   &  (0.005)   &  (0.008)   &  (0.009)   \\
\addlinespace
Ln(HH Income, 99) x Dum99t05&            &    0.053***&    0.052***&    0.055***&    0.058***\\
               &            &  (0.008)   &  (0.008)   &  (0.012)   &  (0.012)   \\
\addlinespace
Ratio of Labor Force (1989) x Dum91t99&            &    0.049** &    0.066***&    0.057***&    0.030   \\
               &            &  (0.021)   &  (0.023)   &  (0.021)   &  (0.021)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum99t05&            &   -0.192***&   -0.154***&   -0.120***&   -0.109***\\
               &            &  (0.042)   &  (0.043)   &  (0.042)   &  (0.039)   \\
\addlinespace
Ln(Num of HU, 91) x Dum91t99&            &            &    0.042***&    0.033***&    0.030***\\
               &            &            &  (0.011)   &  (0.010)   &  (0.010)   \\
\addlinespace
Ln(Num of HU, 99) x Dum99t05&            &            &   -0.031** &   -0.015   &   -0.010   \\
               &            &            &  (0.014)   &  (0.013)   &  (0.013)   \\
\addlinespace
Housing supply elasticity x Dum91t99&            &            &    0.000   &    0.000   &    0.001   \\
               &            &            &  (0.001)   &  (0.001)   &  (0.001)   \\
\addlinespace
Housing supply elasticity x Dum99t05&            &            &   -0.010***&   -0.009***&   -0.010***\\
               &            &            &  (0.002)   &  (0.002)   &  (0.002)   \\
\addlinespace
House Vacancy Rate (1989) x Dum91t99&            &            &   -0.098***&   -0.093***&   -0.105***\\
               &            &            &  (0.025)   &  (0.024)   &  (0.026)   \\
\addlinespace
House Vacancy Rate (1999) x Dum99t05&            &            &    0.165***&    0.153***&    0.136***\\
               &            &            &  (0.037)   &  (0.038)   &  (0.040)   \\
\addlinespace
Ratio of Renters (1989) x Dum91t99&            &            &   -0.022** &   -0.016   &   -0.001   \\
               &            &            &  (0.010)   &  (0.013)   &  (0.014)   \\
\addlinespace
Ratio of Renters (1999) x Dum99t05&            &            &    0.100***&    0.070** &    0.033   \\
               &            &            &  (0.018)   &  (0.028)   &  (0.029)   \\
\addlinespace
Ratio of Bachelor Educated (1989) x Dum91t99&            &            &            &    0.036** &    0.069***\\
               &            &            &            &  (0.016)   &  (0.024)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum99t05&            &            &            &   -0.052   &   -0.092** \\
               &            &            &            &  (0.035)   &  (0.036)   \\
\addlinespace
Ratio of White Race (1989) x Dum91t99&            &            &            &    0.010   &    0.015   \\
               &            &            &            &  (0.009)   &  (0.009)   \\
\addlinespace
Ratio of White Race (1999) x Dum99t05&            &            &            &    0.005   &   -0.011   \\
               &            &            &            &  (0.015)   &  (0.015)   \\
\addlinespace
Ratio of Immigration (80-90) x Dum91t99&            &            &            &   -0.097***&   -0.135***\\
               &            &            &            &  (0.037)   &  (0.038)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum99t05&            &            &            &    0.287***&    0.380***\\
               &            &            &            &  (0.077)   &  (0.076)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1989) x Dum91t99&            &            &            &            &    0.128   \\
               &            &            &            &            &  (0.149)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x Dum99t05&            &            &            &            &    0.526***\\
               &            &            &            &            &  (0.193)   \\
\addlinespace
Ratio of Health Emp (1989) x Dum91t99&            &            &            &            &   -0.253***\\
               &            &            &            &            &  (0.088)   \\
\addlinespace
Ratio of Health Emp (1999) x Dum99t05&            &            &            &            &    0.585***\\
               &            &            &            &            &  (0.133)   \\
\addlinespace
Ratio of College Students (1989) x Dum91t99&            &            &            &            &   -0.121*  \\
               &            &            &            &            &  (0.064)   \\
\addlinespace
Ratio of College Students (1999) x Dum99t05&            &            &            &            &    0.010   \\
               &            &            &            &            &  (0.053)   \\
\midrule
Obs            &     1344   &     1344   &     1198   &     1198   &     1198   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
KP F-Stat (91-99, Non-Stack Sample)      &    36.95   &    30.94   &    30.94   &    29.57   &    29.87   \\
MOP F-Stat (91-99, Non-Stack Sample)  &    36.55   &    30.87   &    30.87   &    29.53   &    29.76   \\
KP F-Stat (99-05, Non-Stack Sample)       &    26.48   &    25.81   &    16.95   &    17.03   &    17.36   \\
MOP F-Stat (99-05, Non-Stack Sample) &    26.25   &    25.58   &    16.78   &    16.91   &    17.21   \\
CoefEqual\_Chi2 &   12.209   &    8.623   &    6.813   &    6.734   &    6.827   \\
CoefEqual\_PValue&    0.000   &    0.003   &    0.009   &    0.009   &    0.009   \\
\bottomrule




\end{tabular}

} % end of resize box

\end{table}

==> Table/table_HPI.D91t99vsD99t05.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D91t99vsD99t05.PLNJM.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of House Price Growth on PLNJM Growth in Prior (91-99) and Boom (99-05) Periods} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{91,99} \& \triangle_{99,05} Ln(HPI_{c}) = \beta_{91,99} * \triangle_{91,99} Ln(PLNJM_{c}) \times Dum_{91,99} + \beta_{99,05} * \triangle_{99,05} Ln(PLNJM_{c}) \times Dum_{99,05} + \gamma_{91,99}* \bm{Controls_{c}} \times Dum_{91,99} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05}  + \alpha_{91,99} + \alpha_{99,05} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{91,99} \& \triangle_{99,05} Ln(HPI_{c})$ is the stacked growth rate of house price index at county $c$ 91-99 and 99-05. The key variable of interest $\triangle_{91,99} Ln(PLNJM_{c})$ and $\triangle_{99,05} Ln(PLNJM_{c})$ are the growth rate of the dollar amount of private-label (non-jumbo) mortgages at county $c$ 91-99 and 99-05, respectively. $Controls_{c}$ indicates control variables at county $c$ in the period start year either 1991 or 1999. We use the gravity model-based instrumental variable $\triangle_{91,99}\text{givNetExp}_{m}$ and $\triangle_{99,05}\text{givNetExp}_{m}$ as IVs for $\triangle_{91,99}Ln(PLNJM_{c})$ and $\triangle_{99,05}Ln(PLNJM_{c})$. Regression is weighted by the natural logarithm of housing units in the start year (either 1991 or 1999). We report the statistics and p-values for the tests of coefficient equality between $\beta_{91,99}$ and $\beta_{99,05}$. For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. We report Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_HPI.D91t99vsD99t05.PLNJM.2SLS}


\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{House Price Growth (91-99 \& 99-05, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
PLNJM Growth (NumLoan, 91-99, An)&   -0.335   &   -0.384   &   -0.366   &   -0.384   &    0.825   \\
               &  (0.525)   &  (0.635)   &  (0.650)   &  (0.698)   &  (2.084)   \\
\addlinespace
PLNJM Growth (NumLoan, 99-05, An)&    0.616** &    0.503** &    0.360***&    0.367***&    0.309** \\
               &  (0.253)   &  (0.225)   &  (0.131)   &  (0.133)   &  (0.151)   \\
\addlinespace
Dummry 91-99   &    0.070   &    0.044   &   -0.007   &   -0.092   &   -0.309   \\
               &  (0.077)   &  (0.052)   &  (0.170)   &  (0.077)   &  (0.567)   \\
\addlinespace
Dummry 99-05   &   -0.026   &   -0.152***&   -0.828***&   -0.897***&   -0.522*  \\
               &  (0.027)   &  (0.037)   &  (0.282)   &  (0.292)   &  (0.283)   \\
\addlinespace
Ln(Num of HH, 92) x Dum92t02&            &    0.003   &    0.003   &   -0.032   &    0.063   \\
               &            &  (0.004)   &  (0.005)   &  (0.047)   &  (0.177)   \\
\addlinespace
Ln(Num of HH, 02) x Dum02t06&            &    0.012***&    0.008***&   -0.015   &   -0.016   \\
               &            &  (0.003)   &  (0.003)   &  (0.015)   &  (0.016)   \\
\addlinespace
Ln(HH Income, 92) x Dum92t02&            &            &    0.005   &    0.013** &    0.024   \\
               &            &            &  (0.012)   &  (0.006)   &  (0.035)   \\
\addlinespace
Ln(HH Income, 02) x Dum02t06&            &            &    0.069** &    0.074***&    0.044*  \\
               &            &            &  (0.027)   &  (0.028)   &  (0.025)   \\
\addlinespace
Ln(Num of HU, 92) x Dum92t02&            &            &            &    0.035   &   -0.068   \\
               &            &            &            &  (0.053)   &  (0.189)   \\
\addlinespace
Ln(Num of HU, 02) x Dum02t06&            &            &            &    0.024*  &    0.022   \\
               &            &            &            &  (0.014)   &  (0.015)   \\
\addlinespace
Housing supply elasticity x Dum92t02&            &            &            &            &    0.006   \\
               &            &            &            &            &  (0.020)   \\
\addlinespace
Housing supply elasticity x Dum02t06&            &            &            &            &   -0.011***\\
               &            &            &            &            &  (0.003)   \\
\midrule
Obs            &     1382   &     1382   &     1382   &     1382   &     1230   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
Kleibergen-Paap F-Stat (91-99, Non-Stack Sample)      &    0.715   &    0.563   &    0.496   &    0.456   &    0.143     \\
MOP F-Eff (91-99, Non-Stack Sample)  &    0.661   &    0.521   &    0.459   &    0.419   &    0.134   \\
Kleibergen-Paap F-Stat (99-05, Non-Stack Sample)       &    9.079   &    10.05   &    17.62   &    17.70   &    13.50   \\
MOP F-Eff (99-05, Non-Stack Sample) &    8.880   &    9.802   &    17.05   &    17.10   &    13.05   \\
CoefEqual\_Chi2 &    2.867   &    1.759   &    1.176   &    1.110   &    0.061   \\
CoefEqual\_PValue&    0.090   &    0.185   &    0.278   &    0.292   &    0.805   \\
\bottomrule




\end{tabular}

} % end of resize box

\end{table}

==> Table/table_HPI.D91t99vsD99t05.PLMNJ.4Reg.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D91t99vsD99t05.PLNJM.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Stacked Regressions of House Price Growth on PLNJM Growth in Prior (91-99) and Boom (99-05) Periods} \smallskip \newline
{\scriptsize
This table reports OLS, reduced-form, first stage, and second stages of stacked 2SLS regression $\triangle_{91,99} \& \triangle_{99,05} Ln(HPI_{c}) = \beta_{91,99} * \triangle_{91,99} Ln(PLNJM_{c}) \times Dum_{91,99} + \beta_{99,05} * \triangle_{99,05} Ln(PLNJM_{c}) \times Dum_{99,05} + \gamma_{91,99}* \bm{Controls_{c}} \times Dum_{91,99} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05}  + \alpha_{91,99} + \alpha_{99,05} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{91,99} \& \triangle_{99,05} Ln(HPI_{c})$ is the stacked growth rate of house price index at county $c$ 91-99 and 99-05. The key variable of interest $\triangle_{91,99} Ln(PLNJM_{c})$ and $\triangle_{99,05} Ln(PLNJM_{c})$ are the growth rate of the dollar amount of private-label (non-jumbo) mortgages at county $c$ 91-99 and 99-05, respectively. $Controls_{c}$ indicates control variables at county $c$ in the period start year either 1991 or 1999. We use the gravity model-based instrumental variable $\triangle_{91,99}\text{givNetExp}_{m}$ and $\triangle_{99,05}\text{givNetExp}_{m}$ as IVs for $\triangle_{91,99} Ln(PLNJM_{c}$ and $\triangle_{99,05}Ln(PLNJM_{c})$. Each regression is weighted by the natural logarithm of housing units in the start year (either 1991 or 1999). For the first-stage F-test of the non-stacked sample, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_HPI.D91t99vsD99t05.PLNJM.4Reg}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{l*{6}{c}}
\toprule
Dep Var (Panel A, B, and C)                      &\multicolumn{5}{c}{House Price Growth (91-99 \& 99-05, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\     


\midrule
\multicolumn{6}{l}{\textbf{Panel A. OLS estimates}} \\
Net Export Growth (91-99, An)&   -0.775   &   -0.415   &   -0.277   &   -0.277   &    0.434   \\
               &  (0.995)   &  (0.976)   &  (0.935)   &  (0.944)   &  (0.989)   \\
\addlinespace
Net Export Growth (99-05, An)&    4.508***&    4.028***&    3.791***&    3.779***&    1.930** \\
               &  (0.994)   &  (0.959)   &  (0.875)   &  (0.890)   &  (0.751)   \\
\addlinespace
R2-adj         &    0.563   &    0.611   &    0.624   &    0.629   &    0.684   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel B. Reduced-form estimates}} \\
GIV Net Export Growth (91-99, An)&   -3.711** &   -3.642** &   -3.677** &   -3.677** &   -3.142*  \\
               &  (1.551)   &  (1.587)   &  (1.572)   &  (1.573)   &  (1.671)   \\
\addlinespace
GIV Net Export Growth (99-05, An)&    7.677***&    6.886***&    6.428***&    6.819***&    4.968***\\
               &  (1.967)   &  (2.062)   &  (1.960)   &  (1.946)   &  (1.396)   \\
\addlinespace
R2-adj         &    0.559   &    0.609   &    0.621   &    0.628   &    0.688   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
PLNJM Growth (91-99, An) x Dum92t02 &   -0.335   &   -0.384   &   -0.366   &   -0.384   &    0.825   \\
               &  (0.525)   &  (0.635)   &  (0.650)   &  (0.698)   &  (2.084)   \\
\addlinespace
PLNJM Growth (99-05, An) x Dum02t06 &    0.616** &    0.503** &    0.360***&    0.367***&    0.309** \\
               &  (0.253)   &  (0.225)   &  (0.131)   &  (0.133)   &  (0.151)   \\
\addlinespace
\addlinespace

Dep Var (Panel D): &\multicolumn{5}{c}{PLNJM Growth (91-99, An)} \\ 
\midrule 
\multicolumn{6}{l}{\textbf{Panel D . First-stage estimates only for 91-99 (non-stack sample)}} \\
\addlinespace
GIV NEG (91-99, An) &    3.150   &    2.842   &    2.668   &    2.568   &   -1.455   \\
               &  (3.726)   &  (3.789)   &  (3.790)   &  (3.802)   &  (3.853)   \\
\addlinespace
Kleibergen-Paap F-Stat      &    0.715   &    0.563   &    0.496   &    0.456   &    0.143   \\
MOP F-Eff &    0.661   &    0.521   &    0.459   &    0.419   &    0.134   \\

\addlinespace
\addlinespace

Dep Var (Panel E): &\multicolumn{5}{c}{PLNJM Growth (99-05, An)} \\ 
\midrule 
\multicolumn{6}{l}{\textbf{Panel E . First-stage estimates only for 99-05 (non-stack sample)}} \\
\addlinespace
GIV NEG (99-05, An) &    9.987***&   10.309***&   13.663***&   13.674***&   11.336***\\
               &  (3.314)   &  (3.252)   &  (3.255)   &  (3.251)   &  (3.085)   \\
\addlinespace
Kleibergen-Paap F-Stat      &    9.079   &    10.05   &    17.62   &    17.70   &    13.50   \\
MOP F-Eff &    8.880   &    9.802   &    17.05   &    17.10   &    13.05   \\

\midrule
\multicolumn{6}{l}{\textbf{Controls (for all Panels)}} \\
DumPeriod  &    Y        &  Y   &   Y    & Y    &  Y    \\
Basic Controls x DumPeriod &            &  Y   &   Y    & Y    &  Y    \\
Housing Controls x DumPeriod &           &      & Y       & Y    &  Y    \\
Demographic Controls x DumPeriod &            &      &        &  Y    &  Y    \\
Industry Controls x DumPeriod &            &      &        &      &  Y    \\

\midrule              
Obs (Panel A, B, and C)          &     1382   &     1382   &     1382   &     1382   &     1230   \\
Obs (Panel D and E)           &      691   &      691   &      691   &      691   &      615   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
\bottomrule
\end{tabular}

} % end of resize box

\end{table}


==> Table/table_HPI.D99t05.2SLS.tex <==
%-----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Regression of House Price Growth on Net Export Growth in Boom Period (99-05)} \smallskip \newline
{\footnotesize 
This table reports 2SLS regression $\triangle_{99,05} Ln(HPI_{c}) = \beta * \triangle_{99,05} \text{NetExp}_{m} + \gamma* \bm{Controls_{c}} + \alpha + \epsilon_{c}$. The left-hand-side dependent variable $\triangle_{99,05} Ln(HPI_{c})$ is the growth rate of the house price index at county $c$ 99-05, and the key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in 1999. We use the gravity model-based instrumental variable ($\triangle_{99,05}\text{givNetExp}_{m}$) as IV for $\triangle_{99,05}\text{NetExp}_{m}$. For the first-stage F-test, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Regression is weighted by the natural logarithm of housing units in 1999. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
\smallskip \newline
} % end of caption
\label{table_HPI.D99t05.2SLS}

\resizebox{\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
            &\multicolumn{5}{c}{House Price Growth (1999-2005, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An)&    6.468***&    5.635** &    5.378** &    5.367** &    3.482** \\
               &  (2.379)   &  (2.389)   &  (2.241)   &  (2.259)   &  (1.618)   \\
\addlinespace
Ln(Num of HH, 02)&            &    0.009***&    0.008***&   -0.028** &   -0.034***\\
               &            &  (0.002)   &  (0.003)   &  (0.013)   &  (0.013)   \\
\addlinespace
Ln(HH Income, 02)&            &            &    0.012   &    0.020*  &   -0.001   \\
               &            &            &  (0.013)   &  (0.012)   &  (0.009)   \\
\addlinespace
Ln(Num of HU, 02)&            &            &            &    0.037***&    0.040***\\
               &            &            &            &  (0.014)   &  (0.013)   \\
\addlinespace
Housing supply elasticity&            &            &            &            &   -0.015***\\
               &            &            &            &            &  (0.002)   \\
\midrule
Obs            &      788   &      788   &      788   &      788   &      697   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   \\
CD F-Stat      &    498.9   &    487.1   &    470.7   &    470.4   &    363.4   \\
Kleibergen-Paap F-Stat      &    25.21   &    24.78   &    24.03   &    24.11   &    17.18   \\
MOP F-Eff&    24.82   &    24.39   &    23.64   &    23.74   &    16.94   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table/table_HPI.D99t05.4Reg.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D99t05.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Regressions of House Price Growth on Net Export Growth in Boom Period (99-05)} \smallskip \newline
{\footnotesize 
This table reports OLS, reduced-form, first stage, and second stage results of 2SLS regression $\triangle_{99,05} Ln(HPI_{c}) = \beta * \triangle_{99,05} \text{NetExp}_{m} + \gamma* \bm{Controls_{c}} + \alpha + \epsilon_{c}$. The left-hand-side dependent variable $\triangle_{99,05} Ln(HPI_{c})$ is the growth rate of the house price index at county $c$ 99-05, and the key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in 1999. We use the gravity model-based instrumental variable ($\triangle_{99,05}\text{givNetExp}_{m}$) as IV for $\triangle_{99,05}\text{NetExp}_{m}$. For the first-stage F-test, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Each regression is weighted by the natural logarithm of housing units in 1999. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_HPI.D99t05.4Reg}



\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
Dep Var (Panel A, B, and C)                     &\multicolumn{5}{c}{House Price Growth (1999-2005, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
\multicolumn{6}{l}{\textbf{Panel A. OLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An)&    6.206***&    5.592***&    5.429***&    5.373***&    4.105***\\
               &  (1.440)   &  (1.425)   &  (1.347)   &  (1.361)   &  (0.861)   \\
\addlinespace
R2-adj         &   0.0818   &    0.139   &    0.141   &    0.149   &    0.309   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel B. Reduced-form estimates}} \\
\addlinespace
GIV Net Export Growth (99-05, An)&    6.133***&    5.295** &    5.000***&    4.989***&    3.143** \\
               &  (1.966)   &  (2.046)   &  (1.876)   &  (1.876)   &  (1.474)   \\
\addlinespace
R2-adj         &   0.0338   &   0.0982   &    0.102   &    0.111   &    0.280   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An)&    6.468***&    5.635** &    5.378** &    5.367** &    3.482** \\
               &  (2.379)   &  (2.389)   &  (2.241)   &  (2.259)   &  (1.618)   \\
\addlinespace 



\addlinespace
\addlinespace


Dep Var (Panel D): &\multicolumn{5}{c}{Net Export Growth (99-05, An)} \\ 
\midrule 
\multicolumn{6}{l}{\textbf{Panel D . First-stage estimates}} \\
\addlinespace
GIV Net Export Growth (99-05, An)&    0.948***&    0.940***&    0.930***&    0.930***&    0.903***\\
               &  (0.189)   &  (0.189)   &  (0.189)   &  (0.189)   &  (0.218)   \\
\addlinespace
Kleibergen-Paap F-Stat      &    25.21   &    24.78   &    24.03   &    24.11   &    17.18   \\
MOP F-Eff&    24.82   &    24.39   &    23.64   &    23.74   &    16.94   \\
\addlinespace
\midrule
\multicolumn{6}{l}{\textbf{Controls (for all Panels)}} \\
Basic Controls &            &  Y   &   Y    & Y    &  Y    \\
Housing Controls &           &      & Y       & Y    &  Y    \\
Demographic Controls &            &      &        &  Y    &  Y    \\
Industry Controls &            &      &        &      &  Y    \\
\midrule              
Obs            &      788   &      788   &      788   &      788   &      697   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_HPI.D99t05vsD07t09.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D99t05vsD07t09.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Housing Price Growth in Boom (99-06) and Bust (07-09) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{99,05} \& \triangle_{07,09} Ln(HPI_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{07,09} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{07,09} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{07,09}* \bm{Controls_{c}} \times Dum_{07,09}  + \alpha_{99,05} + \alpha_{07,09} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{07,09} Ln(HPI_{c})$ is the stacked growth rate of house price index at county $c$ 99-05 and 07-09. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in the start year (either 1999 or 2007).  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_HPI.D99t05vsD07t09.2SLS}


\resizebox{0.52\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{Housing Price Growth (99-05 and 07-09, Annualized )} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum02t06&    6.468***&    5.635** &    5.378** &    5.367** &    3.482** \\
               &  (2.379)   &  (2.389)   &  (2.241)   &  (2.259)   &  (1.618)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum07t09&   -9.338***&   -7.622** &   -7.295** &   -7.258** &   -5.680** \\
               &  (3.268)   &  (3.020)   &  (2.967)   &  (2.971)   &  (2.435)   \\
\addlinespace
Dum02t06   &    0.052***&   -0.047*  &   -0.170   &   -0.261** &    0.022   \\
               &  (0.006)   &  (0.028)   &  (0.119)   &  (0.114)   &  (0.101)   \\
\addlinespace
Dum07t09   &   -0.071***&    0.130***&    0.236** &    0.252** &   -0.019   \\
               &  (0.007)   &  (0.039)   &  (0.116)   &  (0.116)   &  (0.119)   \\
\addlinespace
Ln(Num of HH, 02) x Dum02t06&            &    0.009***&    0.008***&   -0.028** &   -0.034***\\
               &            &  (0.002)   &  (0.003)   &  (0.013)   &  (0.013)   \\
\addlinespace
Ln(Num of HH, 07) x Dum07t09&            &   -0.018***&   -0.017***&    0.012   &    0.038   \\
               &            &  (0.003)   &  (0.004)   &  (0.042)   &  (0.037)   \\
\addlinespace
Ln(HH Income, 02) x Dum02t06&            &            &    0.012   &    0.020*  &   -0.001   \\
               &            &            &  (0.013)   &  (0.012)   &  (0.009)   \\
\addlinespace
Ln(HH Income, 07) x Dum07t09&            &            &   -0.010   &   -0.012   &    0.008   \\
               &            &            &  (0.012)   &  (0.012)   &  (0.011)   \\
\addlinespace
Ln(Num of HU, 02) x Dum02t06&            &            &            &    0.037***&    0.040***\\
               &            &            &            &  (0.014)   &  (0.013)   \\
\addlinespace
Ln(Num of HU, 07) x Dum07t09&            &            &            &   -0.029   &   -0.053   \\
               &            &            &            &  (0.044)   &  (0.037)   \\
\addlinespace
Housing supply elasticity x Dum02t06&            &            &            &            &   -0.015***\\
               &            &            &            &            &  (0.002)   \\
\addlinespace
Housing supply elasticity x Dum07t09&            &            &            &            &    0.016***\\
               &            &            &            &            &  (0.003)   \\
\midrule
Obs            &     1576   &     1576   &     1576   &     1576   &     1394   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
Kleibergen-Paap F-Stat (99-05, non-stack sample)       &    25.21   &    24.78   &    24.03   &    24.11   &    17.18   \\
MOP F-Eff (99-05, non-stack sample)  &    24.82   &    24.39   &    23.64   &    23.74   &    16.94   \\
CoefEqual\_Chi2 &    8.873   &    6.806   &    6.826   &    6.674   &    7.062   \\
CoefEqual\_PValue&    0.003   &    0.009   &    0.009   &    0.010   &    0.008   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table/table_HPI.D99t05vsD07t09.4Reg.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D99t05vsD07t09.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Stacked Regressions of Housing Price Growth in Boom (99-06) and Bust (07-09) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports OLS, reduced-form, first stage, and second stages of stacked 2SLS regression $\triangle_{99,05} \quad \& \quad \triangle_{07,09} Ln(HPI_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{07,09} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{07,09} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{07,09}* \bm{Controls_{c}} \times Dum_{07,09}  + \alpha_{99,05} + \alpha_{07,09} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{07,09} Ln(HPI_{c})$ is the stacked growth rate of house price index at county $c$ 99-05 and 07-09. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}\text{NetExp}_{m}$. Each regression is weighted by the natural logarithm of housing units in the start year 1999. For the first-stage F-test of two non-stacked samples, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_HPI.D99t05vsD07t09.4Reg}
\resizebox{0.82\columnwidth}{!}{%
\begin{tabular}{l*{6}{c}}
\toprule
Dep Var (Panel A, B, and C)                      &\multicolumn{5}{c}{Housing Price Growth (99-05 \& 07-09, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\     


\midrule
\multicolumn{6}{l}{\textbf{Panel A. OLS estimates}} \\
NEG (99-05, An) x Dum02t06&    6.206***&    5.592***&    5.429***&    5.373***&    4.105***\\
               &  (1.440)   &  (1.425)   &  (1.348)   &  (1.362)   &  (0.861)   \\
\addlinespace
NEG (99-05, An) x Dum07t09&   -4.945***&   -3.592***&   -3.216** &   -3.198** &   -1.800*  \\
               &  (1.467)   &  (1.369)   &  (1.292)   &  (1.305)   &  (0.985)   \\
\addlinespace
R2-adj         &    0.536   &    0.582   &    0.583   &    0.584   &    0.642   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel B. Reduced-form estimates}} \\
GIV NEG (99-05, An) x Dum02t06&    6.133***&    5.295** &    5.000***&    4.989***&    3.143** \\
               &  (1.967)   &  (2.047)   &  (1.877)   &  (1.877)   &  (1.475)   \\
\addlinespace
GIV NEG (99-05, An) x Dum07t09&   -8.856***&   -7.155***&   -6.691***&   -6.656***&   -5.074***\\
               &  (2.238)   &  (2.194)   &  (2.068)   &  (2.083)   &  (1.692)   \\
\addlinespace
R2-adj         &    0.532   &    0.578   &    0.580   &    0.581   &    0.641   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
NEG (99-05, An) x Dum02t06&    6.468***&    5.635** &    5.378** &    5.367** &    3.482** \\
               &  (2.379)   &  (2.389)   &  (2.241)   &  (2.259)   &  (1.618)   \\
\addlinespace
NEG (99-05, An) x Dum07t09&   -9.338***&   -7.622** &   -7.295** &   -7.258** &   -5.680** \\
               &  (3.268)   &  (3.020)   &  (2.967)   &  (2.971)   &  (2.435)   \\
\addlinespace
\addlinespace

Dep Var (Panel D): &\multicolumn{5}{c}{Net Export Growth (99-05, An)} \\ 
\midrule 
\multicolumn{6}{l}{\textbf{Panel D . First-stage estimates only for 99-05 (Non-stack sample)}} \\
\addlinespace
NEG (99-05, An) &    6.468***&    5.635** &    5.378** &    5.367** &    3.482** \\
               &  (2.379)   &  (2.389)   &  (2.241)   &  (2.259)   &  (1.618)   \\
\addlinespace
Kleibergen-Paap F-Stat       &    25.21   &    24.78   &    24.03   &    24.11   &    17.18   \\
MOP F-Eff&    24.82   &    24.39   &    23.64   &    23.74   &    16.94   \\
\addlinespace



\midrule
\multicolumn{6}{l}{\textbf{Controls (for all Panels)}} \\
Basic Controls x Dum &            &  Y   &   Y    & Y    &  Y    \\
Housing Controls x Dum &           &      & Y       & Y    &  Y    \\
Demographic Controls x Dum &            &      &        &  Y    &  Y    \\
Industry Controls x Dum &            &      &        &      &  Y    \\
\midrule              
Obs (Panel A, B, and C)          &     1576   &     1576   &     1576   &     1576   &     1394   \\
Obs (Panel D)            &      788   &      788   &      788   &      788   &      697   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU99)}   & {\scriptsize Ln(HU99)}   &{\scriptsize Ln(HU99)}   &{\scriptsize Ln(HU99)}   &{\scriptsize Ln(HU99)}    \\
\bottomrule
\end{tabular}

} % end of resize box

\end{table}


==> Table/table_HPI.D99t05vsD07t09.PLNJM.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D99t05vsD07t09.PLNJM.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Housing Price Growth in Boom (99-05) and Bust (07-09) Periods on PLNJM Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{99,05} \& \triangle_{07,09} Ln(HPI_{c}) = \beta_{99,05} * \triangle_{99,05} Ln(PLNJM_{c}) \times Dum_{99,05} + \beta_{07,09} * \triangle_{99,05} Ln(PLNJM_{c}) \times Dum_{07,09} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{07,09}* \bm{Controls_{c}} \times Dum_{07,09} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{07,09} Ln(HPI_{c})$ is the stacked growth rate of the house price index at county $c$ 99-05 and 07-09. The key variable of interest $\triangle_{99,05} Ln(PLNJM_{c})$ is the growth rate of the dollar amount of private-label (non-jumbo) mortgages at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLNJM_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_HPI.D99t05vsD07t09.PLNJM.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{Housing Price Growth (99-05 and 07-09, Annualized )} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
{\large PLNJM Growth (07USD, 99-05, An) x Dum99t05 } &    {\large 0.500***}&    {\large 0.438***}&    {\large 0.390***}&    {\large 0.432***}&    {\large 0.438***}\\
               &  {\large (0.105)}   &  {\large (0.113)}   &  {\large (0.132)}   &  {\large (0.151)}  &  {\large (0.167)}   \\
\addlinespace
{\large PLNJM Growth (07USD, 99-05, An) x Dum07t09} &   {\large -0.901***}&   {\large -0.830***}&   {\large -0.804***}&   {\large -0.844***}&   {\large -0.896***}\\
               &  {\large (0.209)}  &  {\large (0.211)}  &  {\large (0.273)}   &  {\large (0.261)}  &  {\large (0.293)}   \\
\addlinespace
Dum99t05       &   -0.046***&   -0.546***&   -0.532***&   -0.256*  &   -0.286*  \\
               &  (0.018)   &  (0.127)   &  (0.107)   &  (0.153)   &  (0.153)   \\
\addlinespace
Dum07t09       &    0.099***&    0.594***&    0.440** &    0.726** &    0.778** \\
               &  (0.035)   &  (0.171)   &  (0.208)   &  (0.308)   &  (0.328)   \\
\addlinespace
Ln(Num of HH, 99) x DumD99t05&            &    0.004*  &    0.031** &    0.027*  &    0.025   \\
               &            &  (0.002)   &  (0.016)   &  (0.016)   &  (0.016)   \\
\addlinespace
Ln(Num of HH, 99) x DumD07t09&            &   -0.009***&   -0.070** &   -0.027   &   -0.026   \\
               &            &  (0.003)   &  (0.028)   &  (0.027)   &  (0.029)   \\
\addlinespace
Ln(HH Income, 99) x DumD99t05&            &    0.054***&    0.058***&    0.033** &    0.035** \\
               &            &  (0.012)   &  (0.011)   &  (0.015)   &  (0.015)   \\
\addlinespace
Ln(HH Income, 99) x DumD07t09&            &   -0.055***&   -0.047** &   -0.076** &   -0.080** \\
               &            &  (0.017)   &  (0.021)   &  (0.030)   &  (0.031)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD99t05&            &   -0.163***&   -0.174***&   -0.171***&   -0.165***\\
               &            &  (0.042)   &  (0.050)   &  (0.053)   &  (0.051)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD07t09&            &    0.269***&    0.341***&    0.251***&    0.239***\\
               &            &  (0.055)   &  (0.071)   &  (0.072)   &  (0.080)   \\
\addlinespace
Ln(Num of HU, 99) x DumD99t05&            &            &   -0.035** &   -0.032** &   -0.031*  \\
               &            &            &  (0.016)   &  (0.016)   &  (0.017)   \\
\addlinespace
Ln(Num of HU, 99) x DumD07t09&            &            &    0.064** &    0.024   &    0.023   \\
               &            &            &  (0.029)   &  (0.028)   &  (0.031)   \\
\addlinespace
Housing supply elasticity x DumD99t05&            &            &   -0.005** &   -0.004   &   -0.005*  \\
               &            &            &  (0.002)   &  (0.003)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x DumD07t09&            &            &    0.002   &    0.001   &   -0.000   \\
               &            &            &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
House Vacancy Rate (1999) x DumD99t05&            &            &    0.093** &    0.072   &    0.092** \\
               &            &            &  (0.044)   &  (0.049)   &  (0.043)   \\
\addlinespace
House Vacancy Rate (1999) x DumD07t09&            &            &   -0.017   &    0.021   &    0.055   \\
               &            &            &  (0.083)   &  (0.081)   &  (0.077)   \\
\addlinespace
Ratio of Renters (1999) x DumD99t05&            &            &    0.130***&    0.084***&    0.074** \\
               &            &            &  (0.024)   &  (0.028)   &  (0.038)   \\
\addlinespace
Ratio of Renters (1999) x DumD07t09&            &            &   -0.041   &    0.017   &   -0.001   \\
               &            &            &  (0.052)   &  (0.048)   &  (0.061)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD99t05&            &            &            &    0.066   &    0.024   \\
               &            &            &            &  (0.046)   &  (0.050)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD07t09&            &            &            &    0.165*  &    0.067   \\
               &            &            &            &  (0.090)   &  (0.110)   \\
\addlinespace
Ratio of White Race (1999) x DumD99t05&            &            &            &   -0.001   &   -0.007   \\
               &            &            &            &  (0.014)   &  (0.014)   \\
\addlinespace
Ratio of White Race (1999) x DumD07t09&            &            &            &    0.022   &    0.015   \\
               &            &            &            &  (0.029)   &  (0.030)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD99t05&            &            &            &    0.218** &    0.275***\\
               &            &            &            &  (0.095)   &  (0.100)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD07t09&            &            &            &   -0.562** &   -0.527** \\
               &            &            &            &  (0.219)   &  (0.215)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD99t05&            &            &            &            &   -0.291   \\
               &            &            &            &            &  (0.397)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD07t09&            &            &            &            &   -0.010   \\
               &            &            &            &            &  (0.766)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD99t05&            &            &            &            &    0.363*  \\
               &            &            &            &            &  (0.213)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD07t09&            &            &            &            &    0.332   \\
               &            &            &            &            &  (0.307)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD99t05&            &            &            &            &    0.106   \\
               &            &            &            &            &  (0.147)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD07t09&            &            &            &            &    0.372   \\
               &            &            &            &            &  (0.293)   \\
\addlinespace
Ratio of College Students (1999) x DumD99t05&            &            &            &            &   -0.019   \\
               &            &            &            &            &  (0.063)   \\
\addlinespace
Ratio of College Students (1999) x DumD07t09&            &            &            &            &    0.041   \\
               &            &            &            &            &  (0.130)   \\
\midrule
Obs            &     1572   &     1572   &     1390   &     1390   &     1390   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
KP F-Stat (99-05, non-stack sample)       &    23.08   &    20.62   &    14.24   &    11.79   &    11.22   \\
MOP F-Stat (99-05, non-stack sample)  &    22.02   &    19.84   &    14.40   &    11.90   &    11.20   \\
CoefEqual\_Chi2 &   23.100   &   17.863   &    9.835   &   10.716   &    9.664   \\
CoefEqual\_PValue&    0.000   &    0.000   &    0.002   &    0.001   &    0.002   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table/table_IRSNumHH.D91t07.4Reg.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_IRSNumHH.D92t06.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Regressions of IRS Number of Households Growth (92-06) on Net Export Growth (91-07)} \smallskip \newline
{\footnotesize 
This table reports OLS, reduced-form, first stage and second stage results of 2SLS regression $\triangle_{91,07} Ln(nL\_NumHH_{c}) = \beta * \triangle_{91,07} \text{NetExp}_{m} + \gamma* \bm{Controls_{c}} + \alpha + \epsilon_{c}$. The left-hand-side dependent variable $\triangle_{91,07} Ln(nL\_NumHH_{c})$ is the growth rate of the number of households (filing tax reports) at county $c$ 91-07 and the key variable of interest $\triangle_{91,07} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 91-07. $Controls_{c}$ indicates control variables at county $c$ in 1991. We use the gravity model-based instrumental variable ($\triangle_{91,07}\text{givNetExp}_{m}$) as IV for $\triangle_{912,07}\text{NetExp}_{m}$. For the first-stage F-test, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Each regression is weighted by the natural logarithm of the number of households in 1991. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
\smallskip \newline
} % end of caption
\label{table_IRSNumHH.D92t06.4Reg}



\resizebox{\columnwidth}{!}{%


\begin{tabular}{l*{3}{c}}
\toprule
Dep Var (Panel A, B, and C)                     &\multicolumn{3}{c}{IRS Number of Households Growth (1991-2007, annualized)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
            
\midrule
\multicolumn{4}{l}{\textbf{Panel A. OLS estimates}} \\
\addlinespace
Net Export Growth (91-07, An)&    0.546** &    0.882***&    0.831***\\
               &  (0.232)   &  (0.234)   &  (0.217)   \\
\addlinespace
R2-adj         &  0.00357   &    0.137   &    0.197   \\
\addlinespace


\midrule
\multicolumn{4}{l}{\textbf{Panel B. Reduced-form estimates}} \\
\addlinespace
GIV Net Export Growth (91-07, An)&    0.594*  &    0.881***&    0.807** \\
               &  (0.329)   &  (0.339)   &  (0.338)   \\
\addlinespace
&  0.00168   &    0.131   &    0.192   \\
\addlinespace


\midrule
\multicolumn{4}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (91-07, An)&    0.548*  &    0.827***&    0.762** \\
               &  (0.308)   &  (0.308)   &  (0.315)   \\
\addlinespace 



\addlinespace
\addlinespace


Dep Var (Panel D): &\multicolumn{3}{c}{Net Export Growth (92-06, An)} \\ 
\midrule 
\multicolumn{4}{l}{\textbf{Panel D . First-stage estimates}} \\
\addlinespace
GIV Net Export Growth (91-07, An)&    1.085***&    1.064***&    1.059***\\
               &  (0.117)   &  (0.111)   &  (0.109)   \\
\addlinespace
KP F-Stat      &    86.22   &    91.76   &    93.73   \\
MOP F-Eff      &    86.22   &    91.76   &    93.73   \\

\addlinespace
\midrule
\multicolumn{4}{l}{\textbf{Controls (for all Panels)}} \\
Basic Controls  &            &  Y   &   Y         \\
Demographic Controls  &           &      & Y            \\

\midrule              
Obs            &     1074   &     1074   &     1074   \\   
Cluster SE     &     CBSA   &     CBSA   &     CBSA   \\
Weight         &{\footnotesize Ln(NumHH91)}   &{\footnotesize Ln(NumHH91)}   &{\footnotesize Ln(NumHH91)}     \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}



==> Table/table_PLNJM.D91t99vsD99t05.2SLS.tex <==
%----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PLNJM.D91t99vsD99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of PLNJM Growth in Prior (91-99) and Boom (99-05) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{91,99} \& \triangle_{99,05} Ln(PLNJM_{c}) = \beta_{91,99} * \triangle_{91,99} \text{NetExp}_{m} \times Dum_{91,99} + \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \gamma_{91,99}* \bm{Controls_{c}} \times Dum_{91,99} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05}  + \alpha_{91,99} + \alpha_{99,05} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{91,99} \& \triangle_{99,05} Ln(PLNJM_{c})$ is the stacked growth rate of the dollar amount of private-label (non-jumbo) mortgages (PLNJM) at county $c$ 91-99 and 99-05. The key variable of interest $\triangle_{91,99} \text{NetExp}_{m}$ and $\triangle_{99,05} \text{NetExp}_{m}$ are the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 91-99 and 99-05, respectively. $Controls_{c}$ indicates control variables at county $c$ in the period start year either 1991 or 1999. We use the gravity model-based instrumental variable $\triangle_{91,99}\text{givNetExp}_{m}$ and $\triangle_{99,05}\text{givNetExp}_{m}$ as IVs for $\triangle_{91,99}\text{NetExp}_{m}$ and $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in the start year (either 1991 or 1999). We report the statistics and p-values for the tests of coefficient equality between $\beta_{91,99}$ and $\beta_{99,05}$. For the first-stage F-test of two separate non-stack samples, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_PLNJM.D91t99vsD99t05.2SLS}

\vspace{-2mm}

\resizebox{0.54\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{PLNJM Growth (91-99 and 99-05, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (91-99, An) x Dum91t99&   -2.112   &   -2.461   &   -7.545   &   -7.796*  &   -7.784   \\
               &  (4.200)   &  (4.142)   &  (5.144)   &  (4.562)   &  (4.936)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum99t05&   14.064***&   13.569***&   12.188***&   12.186***&   11.213***\\
               &  (3.571)   &  (3.632)   &  (3.503)   &  (3.539)   &  (3.309)   \\
\addlinespace
Dummry 91-99   &    0.166***&    0.339   &    0.327   &    0.357   &    0.409   \\
               &  (0.009)   &  (0.265)   &  (0.368)   &  (0.536)   &  (0.515)   \\
\addlinespace
Dummry 99-05   &    0.199***&    0.244   &    0.417*  &   -0.371   &   -0.305   \\
               &  (0.009)   &  (0.219)   &  (0.250)   &  (0.401)   &  (0.408)   \\
\addlinespace
Ln(Num of HH, 91) x pd\_D91t99&            &    0.000   &   -0.044   &   -0.107*  &   -0.113** \\
               &            &  (0.004)   &  (0.051)   &  (0.058)   &  (0.049)   \\
\addlinespace
Ln(Num of HH, 99) x pd\_D99t05&            &    0.008***&    0.015   &   -0.007   &   -0.011   \\
               &            &  (0.003)   &  (0.034)   &  (0.033)   &  (0.033)   \\
\addlinespace
Ln(HH Income, 91) x pd\_D91t99&            &   -0.013   &   -0.015   &   -0.003   &   -0.002   \\
               &            &  (0.028)   &  (0.040)   &  (0.056)   &  (0.053)   \\
\addlinespace
Ln(HH Income, 99) x pd\_D99t05&            &   -0.015   &   -0.035   &    0.037   &    0.031   \\
               &            &  (0.024)   &  (0.026)   &  (0.039)   &  (0.039)   \\
\addlinespace
Ratio of Labor Force (1989) x pd\_D91t99&            &   -0.060   &    0.002   &    0.052   &   -0.040   \\
               &            &  (0.101)   &  (0.116)   &  (0.101)   &  (0.104)   \\
\addlinespace
Ratio of Labor Force (1999) x pd\_D99t05&            &    0.027   &    0.103   &    0.160   &    0.156   \\
               &            &  (0.112)   &  (0.101)   &  (0.107)   &  (0.101)   \\
\addlinespace
Ln(Num of HU, 91) x pd\_D91t99&            &            &    0.044   &    0.101*  &    0.108** \\
               &            &            &  (0.051)   &  (0.058)   &  (0.049)   \\
\addlinespace
Ln(Num of HU, 99) x pd\_D99t05&            &            &   -0.003   &    0.020   &    0.024   \\
               &            &            &  (0.035)   &  (0.034)   &  (0.033)   \\
\addlinespace
Housing supply elasticity x pd\_D91t99&            &            &   -0.010***&   -0.007** &   -0.004   \\
               &            &            &  (0.003)   &  (0.003)   &  (0.004)   \\
\addlinespace
Housing supply elasticity x pd\_D99t05&            &            &   -0.011***&   -0.010***&   -0.010***\\
               &            &            &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
House Vacancy Rate (1989) x pd\_D91t99&            &            &    0.267** &    0.182*  &    0.101   \\
               &            &            &  (0.113)   &  (0.104)   &  (0.098)   \\
\addlinespace
House Vacancy Rate (1999) x pd\_D99t05&            &            &    0.156   &    0.164   &    0.102   \\
               &            &            &  (0.106)   &  (0.103)   &  (0.101)   \\
\addlinespace
Ratio of Renters (1989) x pd\_D91t99&            &            &   -0.013   &   -0.202** &   -0.148** \\
               &            &            &  (0.084)   &  (0.079)   &  (0.074)   \\
\addlinespace
Ratio of Renters (1999) x pd\_D99t05&            &            &   -0.109** &   -0.056   &   -0.122** \\
               &            &            &  (0.055)   &  (0.061)   &  (0.062)   \\
\addlinespace
Ratio of Bachelor Educated (1989) x pd\_D91t99&            &            &            &   -0.078   &    0.049   \\
               &            &            &            &  (0.091)   &  (0.105)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D99t05&            &            &            &   -0.263***&   -0.299***\\
               &            &            &            &  (0.096)   &  (0.099)   \\
\addlinespace
Ratio of White Race (1989) x pd\_D91t99&            &            &            &   -0.084*  &   -0.066   \\
               &            &            &            &  (0.046)   &  (0.042)   \\
\addlinespace
Ratio of White Race (1999) x pd\_D99t05&            &            &            &   -0.000   &   -0.023   \\
               &            &            &            &  (0.033)   &  (0.032)   \\
\addlinespace
Ratio of Immigration (80-90) x pd\_D91t99&            &            &            &    1.242***&    1.026***\\
               &            &            &            &  (0.211)   &  (0.254)   \\
\addlinespace
Ratio of Immigration (90-00) x pd\_D99t05&            &            &            &    0.066   &    0.146   \\
               &            &            &            &  (0.191)   &  (0.200)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1989) x pd\_D91t99&            &            &            &            &    0.290   \\
               &            &            &            &            &  (0.473)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x pd\_D99t05&            &            &            &            &    1.774***\\
               &            &            &            &            &  (0.643)   \\
\addlinespace
Ratio of Health Emp (1989) x pd\_D91t99&            &            &            &            &   -1.754***\\
               &            &            &            &            &  (0.525)   \\
\addlinespace
Ratio of Health Emp (1999) x pd\_D99t05&            &            &            &            &    0.527   \\
               &            &            &            &            &  (0.444)   \\
\addlinespace
Ratio of College Students (1989) x pd\_D91t99&            &            &            &            &   -0.298   \\
               &            &            &            &            &  (0.185)   \\
\addlinespace
Ratio of College Students (1999) x pd\_D99t05&            &            &            &            &    0.188   \\
               &            &            &            &            &  (0.166)   \\
\midrule
Obs            &     1404   &     1404   &     1248   &     1248   &     1248   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
KP F-Stat (91-99, Non-stack Sample)     &    45.44   &    46.65   &    34.98   &    33.97   &    34.08   \\
MOP F-Stat (91-99, Non-stack Sample) &    45.60   &    46.92   &    35.74   &    34.65   &    34.74   \\
KP F-Stat (99-05, Non-stack Sample)      &    25.67   &    25.48   &    25.24   &    25.66   &    18.04   \\
MOP F-Stat (99-05, Non-stack Sample) &    23.79   &    23.62   &    16.00   &    16.28   &    16.36   \\
CoefEqual\_Chi2 &    9.642   &    9.165   &    10.24   &    12.32   &    10.54   \\
CoefEqual\_PValue&    0.002   &    0.002   &    0.001   &    0.000   &    0.001   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_PLNJM.D99t05.2SLS.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PLNJM.D99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Regression of PLNJM Growth on Net Export Growth in Boom Period (99-05)} \smallskip \newline
{\footnotesize
This table reports the first-stage and the second-stage results of 2SLS regression $\triangle_{99,05} Ln(PLNJM_{c}) = \beta * \triangle_{99,05} \text{NetExp}_{m} + \gamma* \bm{Controls_{c}} + \alpha + \epsilon_{c}$. The left-hand-side dependent variable $\triangle_{99,05} Ln(PLNJM_{c})$ is the growth rate of the dollar amount of private-label (non-jumbo) mortgages (PLNJM) at county $c$ 99-05 and the key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in 1999. We use the gravity model-based instrumental variable ($\triangle_{99,05}\text{givNetExp}_{m}$) as IV for $\triangle_{99,05}\text{NetExp}_{m}$. For the first-stage F-test, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Regression is weighted by the natural logarithm of housing units in 1999 as the weight for the housing market. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_PLNJM.D99t05.2SLS}



\resizebox{\columnwidth}{!}{%


\begin{tabular}{l*{5}{c}}
\toprule
        &\multicolumn{1}{c}{NEG (99-05, An)}  &\multicolumn{4}{c}{private-label (non-jumbo) mortgages Growth (99-05, 07USD, An)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
GIV Net Export Growth (99-05, An)&    1.142***&            &            &            &            \\
               &  (0.266)   &            &            &            &            \\
\addlinespace
Net Export Growth (99-05, An)&            &   13.694***&   13.365***&   13.049***&   12.851***\\
               &            &  (3.547)   &  (3.643)   &  (3.924)   &  (3.712)   \\
\addlinespace
Ln(Num of households, 1999)&   -0.000   &            &    0.006** &    0.008   &   -0.016   \\
               &  (0.000)   &            &  (0.003)   &  (0.032)   &  (0.033)   \\
\addlinespace
Ln(household Income, 1999)&   -0.002***&            &   -0.004   &   -0.050** &    0.009   \\
               &  (0.001)   &            &  (0.022)   &  (0.025)   &  (0.035)   \\
\addlinespace
Fraction of Labor Force (1999)&   -0.006*  &            &   -0.021   &    0.116   &    0.493***\\
               &  (0.003)   &            &  (0.107)   &  (0.107)   &  (0.144)   \\
\addlinespace
Ln(Num of House Units, 1999)&    0.000   &            &            &    0.001   &    0.023   \\
               &  (0.001)   &            &            &  (0.033)   &  (0.033)   \\
\addlinespace
Housing supply elasticity&   -0.000   &            &            &   -0.004   &   -0.004   \\
               &  (0.000)   &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
Wharton Regulation Index&    0.000** &            &            &    0.022***&    0.020** \\
               &  (0.000)   &            &            &  (0.008)   &  (0.008)   \\
\addlinespace
House Vacancy Rate (1999)&    0.002   &            &            &    0.111   &    0.059   \\
               &  (0.002)   &            &            &  (0.097)   &  (0.093)   \\
\addlinespace
Fraction of Renters (1999)&   -0.001   &            &            &   -0.130** &   -0.104   \\
               &  (0.001)   &            &            &  (0.059)   &  (0.064)   \\
\addlinespace
Fraction of Bachelor Educated (1999)&    0.008***&            &            &            &   -0.296***\\
               &  (0.002)   &            &            &            &  (0.101)   \\
\addlinespace
Fraction of White Race (1999)&    0.001   &            &            &            &   -0.056   \\
               &  (0.001)   &            &            &            &  (0.037)   \\
\addlinespace
Fraction of Immigration (90-00)&   -0.004   &            &            &            &    0.298   \\
               &  (0.003)   &            &            &            &  (0.205)   \\
\addlinespace
Ratio of Age 65 Above (1999)&   -0.011***&            &            &            &    0.638***\\
               &  (0.004)   &            &            &            &  (0.181)   \\
\addlinespace
Constant       &    0.024***&    0.200***&    0.181   &    0.605** &   -0.246   \\
               &  (0.008)   &  (0.009)   &  (0.212)   &  (0.242)   &  (0.359)   \\
\midrule
Obs            &      713   &      792   &      792   &      713   &      713   \\
R2-adj         &    0.413   &   0.0239   &   0.0309   &    0.104   &    0.146   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat      &  18.39          &    23.36   &    23.11   &    16.17   &    18.39   \\
MOP F-Stat     &  18.39          &    23.36   &    23.11   &    16.17   &    18.39   \\
\bottomrule


\end{tabular}

} % end of resize box

\end{table}


==> Table/table_PLNJM.D99t05.4Reg.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PLNJM.D99t05.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Regressions of PLNJM Growth on Net Export Growth in Boom Period (99-05)} \smallskip \newline
{\footnotesize 
This table reports OLS, reduced-form, first stage, and second stage results of 2SLS regression $\triangle_{99,05} Ln(PLNJM_{c}) = \beta * \triangle_{99,05} \text{NetExp}_{m} + \gamma* \bm{Controls_{c}} + \alpha + \epsilon_{c}$. The left-hand-side dependent variable $\triangle_{99,05} Ln(PLNJM_{c})$ is the growth rate of the dollar amount of private-label (non-jumbo) mortgages (PLNJM) at county $c$ 99-05 and the key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in 1999. We use the gravity model-based instrumental variable ($\triangle_{99,05}\text{givNetExp}_{m}$) as IV for $\triangle_{99,05}\text{NetExp}_{m}$. For the first-stage F-test, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Each regression is weighted by the natural logarithm of housing units in 1999. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_PLNJM.D99t05.4Reg}



\resizebox{\columnwidth}{!}{%


\begin{tabular}{l*{4}{c}}
\toprule
Dep Var (Panel A, B, and C)                     &\multicolumn{4}{c}{private-label (non-jumbo) mortgages Growth (07USD, 99-05, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
\multicolumn{5}{l}{\textbf{Panel A. OLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An)&    8.391***&    8.110***&    6.759***&    8.237***\\
               &  (1.551)   &  (1.574)   &  (1.669)   &  (1.863)   \\
\addlinespace
R2-adj         &   0.0406   &   0.0473   &    0.126   &    0.157   \\
\addlinespace


\midrule
\multicolumn{5}{l}{\textbf{Panel B. Reduced-form estimates}} \\
\addlinespace
GIV Net Export Growth (99-05, An)&   15.753***&   15.278***&   14.763***&   14.670***\\
               &  (3.255)   &  (3.331)   &  (3.623)   &  (4.023)   \\
\addlinespace
R2-adj         &   0.0407   &   0.0477   &    0.134   &    0.154   \\
\addlinespace


\midrule
\multicolumn{5}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An)&   13.694***&   13.365***&   13.049***&   12.851***\\
               &  (3.547)   &  (3.643)   &  (3.924)   &  (3.712)   \\
\addlinespace 


\addlinespace
\addlinespace


Dep Var (Panel D): &\multicolumn{4}{c}{Net Export Growth (99-05, An)} \\ 
\midrule 
\multicolumn{5}{l}{\textbf{Panel D . First-stage estimates}} \\
\addlinespace
GIV Net Export Growth (99-05, An)&    1.150***&    1.143***&    1.131***&    1.142***\\
               &  (0.238)   &  (0.238)   &  (0.281)   &  (0.266)   \\
\addlinespace
KP F-Stat      &    23.36   &    23.11   &    16.17   &    18.39   \\
MOP F-Stat     &    23.36   &    23.11   &    16.17   &    18.39   \\
\addlinespace
\midrule
\multicolumn{5}{l}{\textbf{Controls (for all Panels)}} \\
Basic Controls &            &  Y   &   Y    & Y       \\
Housing Controls &           &      & Y       & Y        \\
Demographic Controls &            &      &        &  Y      \\

\midrule              
Obs            &      792   &      792   &      713   &      713   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_PLNJM.D99t05.FirstStage.tex <==
%---------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PLNJM.D99t05.FirstStage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{First-stage Regression Private-label Mortgage Growth 99-05 on Net Export Growth} \smallskip \newline
 Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip \newline
} % end of caption
\label{table_PLNJM.D99t05.FirstStage}

\resizebox{\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
            &\multicolumn{5}{c}{Net Export Growth (1999-2005, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
GIV Net Export Growth (99-05, An)&    0.947***&    0.939***&    0.929***&    0.929***&    0.902***\\
               &  (0.189)   &  (0.189)   &  (0.190)   &  (0.189)   &  (0.217)   \\
\addlinespace
Ln(Num of HH, 02)&            &    0.000   &    0.000   &   -0.000   &   -0.001   \\
               &            &  (0.000)   &  (0.000)   &  (0.000)   &  (0.000)   \\
\addlinespace
Ln(HH Income, 02)&            &            &    0.000*  &    0.001** &    0.001   \\
               &            &            &  (0.000)   &  (0.000)   &  (0.000)   \\
\addlinespace
Ln(Num of HU, 02)&            &            &            &    0.001   &    0.001   \\
               &            &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity&            &            &            &            &   -0.000   \\
               &            &            &            &            &  (0.000)   \\
\midrule
Obs            &      792   &      792   &      792   &      792   &      701   \\
R2-adj         &    0.387   &    0.389   &    0.391   &    0.391   &    0.360   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   & Ln(HU02)   \\
CD F-Stat      &    500.7   &    489.1   &    472.6   &    472.6   &    365.4   \\
Kleibergen-Paap F-Stat      &    25.21   &    24.80   &    24.03   &    24.15   &    17.21   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_PLNJM.D99t05vsD05t08.2SLS.tex <==
%----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PLNJM.D99t05vsD05t08.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of PLNJM Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{99,05} \& \triangle_{05,08} Ln(PLNJM_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(PLNJM_{c})$ is the stacked growth rate of the dollar amount of private-label (non-jumbo) mortgages (PLNJM) at county $c$ 99-05 and 05-08. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ and $\triangle_{05,08} \text{NetExp}_{m}$ are the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05 and 05-08, respectively. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{99,05}$ and $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{05,08} $ as IVs for $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{99,05}$ and $\triangle_{05,08}\text{NetExp}_{m} \times Dum_{05,08} $. Regression is weighted by the natural logarithm of housing units in the start year (either 1999 or 2005). We report the statistics and p-values for the tests of coefficient equality between $\beta_{99,05}$ and $\beta_{05,08}$. For the first-stage F-test of two separate non-stack samples, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_PLNJM.D99t05vsD05t08.2SLS}


\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{PLNJM Growth (99-05 and 05-08, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum99t05&   14.987***&   14.110***&   13.820***&   13.817***&   13.356***\\
               &  (3.582)   &  (3.505)   &  (3.437)   &  (3.412)   &  (3.508)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&  -14.713** &  -13.133** &  -13.704** &  -13.223** &  -10.991** \\
               &  (5.935)   &  (5.994)   &  (6.165)   &  (6.047)   &  (5.062)   \\
\addlinespace
Dummry 99-05   &    0.165***&    0.023   &   -0.203   &   -0.139   &   -0.061   \\
               &  (0.008)   &  (0.047)   &  (0.236)   &  (0.236)   &  (0.255)   \\
\addlinespace
Dummry 05-08   &   -0.394***&   -0.175** &   -0.464   &   -0.573*  &   -1.283***\\
               &  (0.017)   &  (0.075)   &  (0.319)   &  (0.308)   &  (0.326)   \\
\addlinespace
Ln(Num HH, 99) x Dum99t05&            &    0.013***&    0.011***&    0.038   &    0.047*  \\
               &            &  (0.004)   &  (0.003)   &  (0.026)   &  (0.028)   \\
\addlinespace
Ln(Num HH, 05) x Dum05t08&            &   -0.019***&   -0.021***&   -0.082   &   -0.044   \\
               &            &  (0.006)   &  (0.006)   &  (0.067)   &  (0.061)   \\
\addlinespace
Ln(HH Income, 99) x Dum99t05&            &            &    0.023   &    0.017   &    0.012   \\
               &            &            &  (0.020)   &  (0.020)   &  (0.022)   \\
\addlinespace
Ln(HH Income, 05) x Dum05t08&            &            &    0.028   &    0.037   &    0.088***\\
               &            &            &  (0.030)   &  (0.027)   &  (0.029)   \\
\addlinespace
Ln(Num of HH, 99) x Dum99t05&            &            &            &   -0.027   &   -0.037   \\
               &            &            &            &  (0.027)   &  (0.028)   \\
\addlinespace
Ln(Num of HH, 05) x Dum05t08&            &            &            &    0.061   &    0.031   \\
               &            &            &            &  (0.070)   &  (0.064)   \\
\addlinespace
Housing supply elasticity x Dum99t05&            &            &            &            &   -0.007*  \\
               &            &            &            &            &  (0.004)   \\
\addlinespace
Housing supply elasticity x Dum05t08&            &            &            &            &    0.035***\\
               &            &            &            &            &  (0.007)   \\
\midrule
Obs            &     1584   &     1584   &     1584   &     1584   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
Kleibergen-Paap F-Stat (99-05, Non-stack Sample)  &    23.36   &    23.24   &    23.02   &    23.33   &    16.88   \\
MOP F-Eff (99-05, Non-stack Sample) &    22.91   &    22.74   &    22.55   &    22.85   &    16.52   \\
CoefEqual\_Chi2 &   11.758   &    9.916   &    9.720   &    9.722   &   10.102   \\
CoefEqual\_PValue&    0.001   &    0.002   &    0.002   &    0.002   &    0.001   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table/table_PLNJM.D99t05vsD05t08.4Reg.tex <==



%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PLNJM.D99t05vsD05t08.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Stacked Regressions of PLNJM Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports OLS, reduced-form, first stage and second stages of 2SLS stacked regression $\triangle_{99,05} \&  \triangle_{05,08}  Ln(PLNJM_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(PLNJM_{c})$ is the stacked growth rate of the dollar amount of private-label (non-jumbo) mortgages (PLNJM) at county $c$ 99-05 and 05-08. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m} $ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{99,05} $ and $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{05,08} $ as IVs for $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{99,05}$ and $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{05,08}$. Each regression is weighted by the natural logarithm of housing units in the start year (either 1999 or 2005). For the first-stage F-test of two non-stack samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. We report Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_PLNJM.D99t05vsD05t08.4Reg}

\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{l*{6}{c}}
\toprule
Dep Var (Panel A, B, and C)                      &\multicolumn{5}{c}{PLNJM Growth (99-05 \& 05-08, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\     


\midrule
\multicolumn{6}{l}{\textbf{Panel A. OLS estimates}} \\
Net Export Growth (99-05, An) x Dum99t05&    8.858***&    8.260***&    8.048***&    8.115***&    7.044***\\
               &  (1.607)   &  (1.579)   &  (1.521)   &  (1.533)   &  (1.614)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&   -8.150***&   -7.035** &   -7.325** &   -7.183** &   -3.473   \\
               &  (2.968)   &  (2.917)   &  (2.917)   &  (2.877)   &  (2.529)   \\
\addlinespace
R2-adj         &    0.845   &    0.857   &    0.864   &    0.864   &    0.883   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel B. Reduced-form estimates}} \\
GIV Net Export Growth (99-05, An) x Dum99t05&   17.240***&   16.175***&   15.790***&   15.788***&   14.671***\\
               &  (3.307)   &  (3.277)   &  (3.175)   &  (3.193)   &  (3.210)   \\
\addlinespace
GIV Net Export Growth (99-05, An) x Dum05t08&  -16.936***&  -15.033** &  -15.518***&  -15.011***&  -12.101** \\
               &  (5.582)   &  (5.806)   &  (5.838)   &  (5.772)   &  (4.790)   \\
\addlinespace
R2-adj         &    0.860   &    0.864   &    0.865   &    0.865   &    0.879   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An) x Dum99t05&   14.987***&   14.110***&   13.820***&   13.817***&   13.356***\\
               &  (3.582)   &  (3.505)   &  (3.437)   &  (3.412)   &  (3.508)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&  -14.713** &  -13.133** &  -13.704** &  -13.223** &  -10.991** \\
               &  (5.935)   &  (5.994)   &  (6.165)   &  (6.047)   &  (5.062)   \\
\addlinespace
\addlinespace

Dep Var (Panel D): &\multicolumn{5}{c}{Net Export Growth (99-05, An)} \\ 
\midrule 
\multicolumn{6}{l}{\textbf{Panel D . First-stage estimates only for 99-05 (non-stack sample)}} \\
\addlinespace
GIV Net Export Growth (99-05, An)&    1.150***&    1.146***&    1.143***&    1.143***&    1.099***\\
               &  (0.238)   &  (0.238)   &  (0.238)   &  (0.237)   &  (0.267)   \\
\addlinespace
Kleibergen-Paap F-Stat      &    23.36   &    23.24   &    23.02   &    23.33   &    16.88   \\
MOP F-Eff &    22.91   &    22.74   &    22.55   &    22.85   &    16.52   \\

\addlinespace
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Controls (for all Panels)}} \\
Basic Controls x Dum &            &  Y   &   Y    & Y    &  Y    \\
Housing Controls x Dum &           &      & Y       & Y    &  Y    \\
Demographic Controls x Dum &            &      &        &  Y    &  Y    \\
Industry Controls x Dum &            &      &        &      &  Y    \\
\midrule              
Obs (Panel A, B, and C)          &     1584   &     1584   &     1584   &     1584   &     1402   \\
Obs (Panel D)           &      792   &      792   &      792   &      792   &      701   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
\bottomrule
\end{tabular}

} % end of resize box

\end{table}


==> Table/table_ZIP.LMH.HPI.D92t99vsD00t06.PLNJM.4Reg.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_ZIP.LMH.HPI.D92t99vsD00t06.PLNJM.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four stacked Regressions of Low-minus-High House Price Growth on private-label (non-jumbo) mortgages Growth in Prior (92-99) and Boom (00-06)} \smallskip \newline
{\footnotesize 
This table reports OLS, reduced-form, first stage, and second stage results of 2SLS stacked regression $\text{LMH}\triangle_{92,99} \&  \triangle_{00,06} Ln(HPI_{m}) = \beta_{92,99} * \triangle_{92,99} \text{NetExp}_{m} \times Dum_{92,99} + \beta_{00,06} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{00,06} + \gamma_{92,99}* Dum_{92,99} + \gamma_{00,06}* Dum_{00,06} + \epsilon_{period, m}$. The left-hand-side dependent variable $\text{LMH}\triangle_{92,99} \&  \triangle_{00,06} Ln(HPI_{m})$ is the differential growth rate of the house price index at metro $m$ between the low- and high-income ZIP codes 92-99 and 99-05. The dependent variables in column (1) to (4) are the above ``low-minus-high" house price growth based on two, tertile, quartile, and quintile income groups of ZIP codes within metropolitan areas in 1998. The key variable of interest $\text{LMH}\triangle_{92,99} \&  \triangle_{00,06} Ln(HPI_{m})$ is the differential growth rate of the dollar amount (07USD) of private-label (non-jumbo) mortgages (PLNJM) at metro $m$ between the low- and high-income ZIP codes 92-99 and 99-05. We use the gravity model-based instrumental variable ($\triangle_{92,99}\text{givNetExp}_{m}$ and $\triangle_{99,05}\text{givNetExp}_{m}$) as IV for $\triangle_{92,99}\text{NetExp}_{m}$ and $\triangle_{99,05}\text{NetExp}_{m}$. For the first-stage F-test, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Each regression is weighted by the natural logarithm of housing units in metro $m$ in 1992 for 92-99 period and in 1999 for 00-06 period. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively. ``An" means annualized variable. 
} % end of small font size
} % end of caption
\label{table_ZIP.LMH.HPI.D92t99vsD00t06.PLNJM.4Reg}


\resizebox{0.88\columnwidth}{!}{


\begin{tabular}{l*{4}{c}}
\toprule
Dep Var (Panel A, B, and C)                     &\multicolumn{4}{c}{Low-minus-High House Price Growth (92-99 \& 00-06, An, 07USD)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)} \\
            
            &\multicolumn{1}{c}{Two Groups}&\multicolumn{1}{c}{Tertile Groups}&\multicolumn{1}{c}{Quartile Groups}&\multicolumn{1}{c}{Quintile Groups}\\
            
\midrule
\multicolumn{5}{l}{\textbf{Panel A. OLS estimates}} \\
\addlinespace
LMH PLNJM Growth (92-99, An, 07USD) x Dum92t99&    0.008   &    0.003 &    0.003   &    0.002   \\
               &  (0.007)   &  (0.008)   &  (0.010)   &  (0.010)   \\
\addlinespace
LMH PLNJM Growth (99-05, An, 07USD) x Dum00t06&    0.053***  &    0.050*** &    0.048*** &    0.041*** \\
               &  (0.010)   &  (0.014)   &  (0.011)   &  (0.010)   \\
\addlinespace
R2-adj         &    0.126   &    0.115   &    0.120   &    0.109   \\
\addlinespace


\midrule
\multicolumn{5}{l}{\textbf{Panel B. Reduced-form estimates}} \\
\addlinespace
GIV Net Export Growth (92-99, An) x Dum92t99&   -0.219   &   -0.482  &   -0.490  &   -0.602    \\
               &  (0.269)   &  (0.314)   &  (0.377)   &  (0.393)   \\
\addlinespace
GIV Net Export Growth (99-05, An) x Dum00t06&    0.681*  &    1.234***&    1.608***&    1.731***\\
               &  (0.349)   &  (0.465)   &  (0.570)   &  (0.557)   \\
\addlinespace
R2-adj         &   0.0307   &   0.0331   &   0.0438   &   0.0443   \\
\addlinespace


\midrule
\multicolumn{5}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (92-99, An) x Dum92t99&   -0.891   &    0.243   &    -0.418   &    0.268    \\
               &  (15.968)   &  (0.536)   &  (1.384)   &  (0.546)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum99t05&    0.096  &   0.117* &   0.134** &   0.122* \\
               &  (0.060)   &  (0.060)   &  (0.064)   &  (0.063)   \\
\addlinespace
CoefEqual\_Chi2 &    0.004   &    0.058   &    0.161   &    0.077   \\
CoefEqual\_PValue &    0.951   &    0.810   &    0.688   &    0.781   \\

\addlinespace 
\addlinespace


Dep Var (Panel D): &\multicolumn{4}{c}{Low-minus-High PLNJM Growth (92-99, An, 07USD)} \\ 
\midrule 
\multicolumn{5}{l}{\textbf{Panel D . First-stage estimates only for 92-99 (Non-stack sample)}} \\
\addlinespace
GIV Net Export Growth (92-99, An) x Dum92t99&    0.245   &   -1.988   &    1.171   &   -2.244   \\
               &  (4.406)   &  (4.082)   &  (3.973)   &  (3.963)   \\
\addlinespace
KP F-Stat      &  0.00310   &    0.237   &   0.0869   &    0.321   \\
MOP F-Stat     &  0.00310   &    0.237   &   0.0869   &    0.321   \\
\addlinespace
\addlinespace 


Dep Var (Panel E): &\multicolumn{4}{c}{Low-minus-High PLNJM Growth (99-05, An, 07USD)} \\ 
\midrule 
\multicolumn{5}{l}{\textbf{Panel D . First-stage estimates only for 00-06 (Non-stack sample)}} \\
\addlinespace
GIV Net Export Growth (99-05, An) x Dum00t06&    7.090** &   10.554** &   12.028** &   14.173** \\
               &  (3.446)   &  (4.551)   &  (4.820)   &  (6.253)   \\
\addlinespace
KP F-Stat      &    4.233   &    5.379   &    6.228   &    5.138   \\
MOP F-Stat     &    4.233   &    5.379   &    6.228   &    5.138   \\
\addlinespace



\midrule  
Obs (Panel A, B, and C)         &      495   &      495   &      495   &      495   \\
Obs (Panel D)           &      225   &      225   &      225   &      225   \\
Obs (Panel E)          &      270   &      270   &      270   &      270   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA     \\
Weight         &{\scriptsize Ln(CBSAHU,start)}   &{\scriptsize Ln(CBSAHU,start)}   &{\scriptsize Ln(CBSAHU,start)}   &{\scriptsize Ln(CBSAHU,start)}   \\
\bottomrule

\end{tabular}
} % end of resize box

\end{table}


==> Table/table_ZIP.Low-Minus-High.PLMNJ.D99t05.4Reg.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_ZIP.Low-Minus-High.PLNJM.D99t05.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Regressions of Low-minus-High PLNJM Growth on Net Export Growth in Boom Period (99-05} \smallskip \newline
{\footnotesize 
This table reports OLS, reduced-form, first stage, and second stage results of 2SLS regression $\text{LMH}\triangle_{99,05} Ln(PLNJM_{m}) = \beta * \triangle_{99,05} \text{NetExp}_{m} + \alpha + \epsilon_{c}$. The left-hand-side dependent variable $\text{LMH}\triangle_{99,05} Ln(PLNJM_{m})$ is the differential growth rate of the dollar amount of private-label (non-jumbo) mortgages (PLNJM) at metro $m$ between the high-income ZIP codes and low-income ZIP codes 99-05. The key variable of interest $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. We use the gravity model-based instrumental variable ($\triangle_{99,05}\text{givNetExp}_{m}$) as IV for $\triangle_{99,05}\text{NetExp}_{m}$. For the first-stage F-test, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Each regression is weighted by the natural logarithm of housing units in metro $m$ in 1999. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively. ``An" means annualized variable. 
} % end of small font size
} % end of caption
\label{table_ZIP.Low-Minus-High.PLNJM.D99t05.4Reg}


\resizebox{\columnwidth}{!}{


\begin{tabular}{l*{4}{c}}
\toprule
Dep Var (Panel A, B, and C)                     &\multicolumn{4}{c}{Low-minus-High private-label (non-jumbo) mortgage Growth (99-05, An, 07USD)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{Half}&\multicolumn{1}{c}{Tertile}&\multicolumn{1}{c}{Quartile}&\multicolumn{1}{c}{Quintile} \\
            
\midrule
\multicolumn{5}{l}{\textbf{Panel A. OLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An)&  2.679& 4.133    & 4.505*    &5.851*      \\
               &(2.005)      & (2.533)     & (2.602)    &(3.323)       \\
\addlinespace
R2-adj         &0.00141       &0.00353       &0.00425        &0.00539         \\
\addlinespace


\midrule
\multicolumn{5}{l}{\textbf{Panel B. Reduced-form estimates}} \\
\addlinespace
GIV Net Export Growth (99-05, An) &4.037    & 7.139   &10.446*    &12.327*     \\
               &(3.642)     &(4.748)     &(5.440)    &(6.513)       \\
\addlinespace
R2-adj         &0.000155     &0.00324      &0.00952       &0.00886          \\
\addlinespace


\midrule
\multicolumn{5}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An) &4.609   &8.150    &12.074*   &14.248**        \\
               &(4.137)     &(5.351)     &(6.292)     &(7.020)       \\
\addlinespace 


\addlinespace
\addlinespace


Dep Var (Panel D): &\multicolumn{4}{c}{Net Export Growth (99-05, An)} \\ 
\midrule 
\multicolumn{5}{l}{\textbf{Panel D . First-stage estimates}} \\
\addlinespace
GIV Net Export Growth (99-05, An) &0.876***    &0.876***    &0.865***    &0.865***    \\
               &(0.215)     &(0.215)     &(0.226)     &(0.226)         \\
\addlinespace
KP F-Stat      &16.67       &16.67       &14.68      &14.68          \\
MOP F-Stat     &16.39       &16.39       &14.40       &14.40           \\
\addlinespace


\midrule  
Obs            &      311   & 311        & 298        & 298           \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA     \\
Weight         &{\scriptsize Ln(CBSAHU99)}   &{\scriptsize Ln(CBSAHU99)}   &{\scriptsize Ln(CBSAHU99)}   &{\scriptsize Ln(CBSAHU99)}   \\
\bottomrule

\end{tabular}
} % end of resize box

\end{table}

